ProS: Data Series Progressive k-NN Similarity Search and Classification with Probabilistic Quality Guarantees

Existing systems dealing with the increasing volume of data series cannot guarantee interactive response times, even for fundamental tasks such as similarity search. Therefore, it is necessary to develop analytic approaches that support exploration and decision making by providing progressive results, before the final and exact ones have been computed. Prior works lack both efficiency and accuracy when applied to large-scale data series collections. We present and experimentally evaluate ProS, a new probabilistic learning-based method that provides quality guarantees for progressive Nearest Neighbor (NN) query answering. We develop our method for k-NN queries and demonstrate how it can be applied with the two most popular distance measures, namely, Euclidean and Dynamic Time Warping (DTW). We provide both initial and progressive estimates of the final answer that are getting better during the similarity search, as well suitable stopping criteria for the progressive queries. Moreover, we describe how this method can be used in order to develop a progressive algorithm for data series classification (based on a k-NN classifier), and we additionally propose a method designed specifically for the classification task. Experiments with several and diverse synthetic and real datasets demonstrate that our prediction methods constitute the first practical solutions to the problem, significantly outperforming competing approaches. This paper was published in the VLDB Journal (2022).

==> approach-notes.tex <==
% !TEX root = main.tex

\newpage
\section{Older Notes on Proposed Approach}
\label{sec:approach}

Previous work on progressive or optimistic visual analytics~\cite{Fisher:2012, Stolper:2014, Moritz:2017} has focused on the estimation of aggregated functions, such as the mean, over random or carefully selected samples of the data. In this case, providing feedback to users about the uncertainty of progressive results can rely on common statistical methods, e.g., confidence intervals~\cite{Fisher:2012,Moritz:2017}, or coarse-grain visualizations of aggregated data~\cite{Glueck:2014}. 
However, such approaches cannot apply to our problem. Although k-NN distances converge over time (see Fig.~\ref{fig:progressive-answers}), providing bounds for their error requires a different set of statistical tools.   

Our vision is to develop methods for progressive time series similarity search, coupled with appropriate bounds on the errors of the intermediate results.
We are inspired by the probabilistic approach of Ciaccia and Patella~\cite{Ciaccia:2000} on approximate search in multi-dimensional spaces. According to this approach, a dataset is considered as a random sample (or instance) drawn from a large multidimensional space. If the distribution of k-NN distances in this space is known for any given query, then we can derive an estimate of the k-NN distance for the sample. Unfortunately, such distributions are unknown, so the challenge is how to approximate them from a given dataset. 
Ciaccia and Patella~\cite{Ciaccia:2000} use this framework to determine a mix of probability and distance error bounds as stopping conditions for an approximate similarity search. Our goal instead is to provide live estimates of probabilistic distance bounds to users, and let users decide whether to trust the current results and stop, wait for a better answer, or keep the process executing in the background while they continue with a new search. 

We briefly discuss promising measures that could help users evaluate the progressive results of a similarity search. 
Let $\mathcal{T}$ be a space of time series data. 
For a given query $Q \in \mathcal{T}$, we define the cumulative distribution function $F_Q(x) = Pr\{d_Q \leq x\}$ that gives the probability that its distance $d_Q$ from a random series in $\mathcal{T}$ is lower than or equal to $x$. 
From this function, we can derive the probability distribution of k-NN distances $d^{k}_Q$, and from this, we can estimate the expected k-NN distance and assess the uncertainty of this value. 
Furthermore, we can infer probabilistic distance bounds for $d^{k}_Q$. For example, we can estimate a distance bound $d^{+}$ such that $Pr\{d^{k}_Q > d^{+}\} \leq 5\%$. 
The $F_Q$ function can be also used to derive a probability distribution for the number $k$ of answers whose distance is better than a given distance $d_Q$. 
Investigating additional probabilistic measures about expected CPU and I/O costs~\cite{Ciaccia:1998:CMS} can also be useful.

We note that the above directions pose two main challenges. First, the $F_Q(x)$ function can be only approximated based on a specific instance of the space, i.e., the given time series dataset. Ciaccia and Patella~\cite{Ciaccia:2000} argue that for high-dimensional spaces, this function is close to the cumulative distribution function $F(x)$ of all pairwise distances, and can be approximated from a sample of distances that are randomly drawn from a given dataset. Unfortunately, reliably estimating the probability distribution of k-NN distances requires large samples of distances. Our early tests have shown that their precomputation can be prohibitively expensive for large datasets, such as the ones in Table~\ref{tab:datasets}, or larger. We are currently working on solutions that reduce such computation costs. 

The second challenge is how to communicate to users probabilistic distance bounds and errors, given that similarity distance values do not have a clear interpretation. Our goal is to integrate these distance bounds and errors into the visual representation of a time series, by either using the query itself, or its progressive k-NN answers. 
Finally, we are interested in experimentally assessing how users perceive and understand such probabilistic measures. 
We plan to measure whether, and to what extent, the visualization of these probabilistic measures helps them to effectively complete their visual analysis tasks.  

%Let us consider a time series dataset $T$, which consists of multiple time series $t$, and a nearest neighbor query $Q$ over the dataset. We define the distance distribution (d.d.) of the dataset as $F(x) = Pr\{d(t1, t2) \leqslant x\}$ (1) where t1 and t2 are two (independent) random series of the dataset and $d(t1, t2)$ is the distance between them. Given the d.d. of the dataset or a sample of the dataset, we can compute the expected kNN distance, the expected number of better answers from every current, best-so-far (BSF) answer, and the expected CPU and I/O costs of our nearest neighbor queries ~\cite{TODO}. 

%Given a query $Q$ in this space, the authors assume that the distribution of the k-NN distance $d^{k}_Q$ has a probability density function $g^k_Q(x) = Pr\{d^{k}_Q = x\}$. If we know this function, we can estimate the expected k-NN distance and then assess the uncertainty of our estimate. Furthermore, We can derive probabilistic distance bounds for $d^{k}_Q$. For example, we can estimate the upper distance bound $D$ for the k-NN distance such that $Pr\{d^{k}_Q > D\} \leq 5\%$. Finally, we can  

%The main objective of our work is on how to aid users finish their searches much faster. Previous works on progressive visual analytics (see Sec.~\ref{sec:related-work}) don't consider similarity search queries. Only Ciaccia and Patella ~\cite{Ciaccia:2000} proposed a probabilistic approach for the computation of the expected kNN distance and the error of progressive similarity search query answering on multidimensional objects. However, they didn't evaluate their approach with a user study and they didn't use time series data. Thus, we don't know how real users can assimilate this probabilistic information and how this is going to change their data exploration process. Based on the work of Ciaccia and Patela ~\cite{Ciaccia:2000}, we present the design of our future user study where we are going to evaluate whether users are able to assess the quality of progressive results and terminate their exploratory process much faster than the the time it takes to the algorithm to finish the exact search. 

\iffalse
\vspace{5pt} 
\noindent
%\paragraph
\textbf{Expected Number of Better Answers.} Given the d.d. and the current BSF answer with distance r from the query $Q$, we are able to compute the probability that at least $k$ time series have distance from $Q$ less than r: $P_{Q,k}(r) = Pr_k\{d(Q, t) \leqslant r\}$ (2) ~\cite{TODO}. 

\vspace{5pt} 
\noindent
%\paragraph
\textbf{Expected k-NN Distance.} The formula (2), in other words, gives the probability that $d(Q, t)$ is at most r. If we upper bound the distance r with a finite number of distances $d+$, we can compute the expected 1NN distance by integrating the derivative of $P_{Q,k}(r)$ (i.e., the density function) (3) over all r values ~\cite{TODO}.

\vspace{5pt} 
\noindent
%\paragraph
\textbf{Expected I/O and CPU Costs.} Finally, based on the probability that a node at level l is accessed, the number of indexed objects, and the density function (3), we can compute the average number of pages accessed and the average number of distances computed (I/O and CPU costs, respectively). 
\fi

%Previous user studies ~\cite{TODO} examined how users assess the progressive average value and the accompanied error they get from progressive aggregate queries over large relational databases and how this information guides their decision making and exploration process. There is no work on evaluating with users the results of progressive similarity search queries on time series data. In Sec. 3, we demonstrated the need of progressive similarity query answering and how users can be in the loop in order to terminate the search much faster before the end of the algorithm and still not losing in accuracy (or losing accuracy given some guarantees). As such, we are the first to design and run a user study in order to understand which probabilistic information of progressively similar results would be useful to users for rapid decision making and elimination of their waiting times. Even if approximate results converge to the exact one very fast, progressive similarity search is still useful, because the users do not know what the exact answer is until the end of the algorithm, which usually takes time. 

%In our user study, we plan to show the approximate answer to the users quickly, along with an estimation of how close it is to the exact answer, how many better answers they should expect for, as well as the expected I/O and CPU cost of the algorithm till the finish of its execution. Next, we are going to present good candidates a few seconds in (likely 1NN given our results), and progressive afterwards if the user wants it. And here we need to study how often to give updates to the users. 

%\anna{Question on user study: den mporousa na perigrapsw me megaluterh leptomereia to user study, gt de mou einai clear pws 8a kanoume evaluate ta results tou user study, an oi users mas einai non experts}

%Present future steps, i.e., user study to be done, and OPEN research problems (vis: visualizations/interaction with users, databases: scalability of methods). 











\subsection{baseline}

patella approaches: with/without witnesses

without witnesses: we estimate the result of every query using the same overall distr (compute all pair wise distances of a sample of the dataset, produce distr of these distances: F(x), use this distr to produce the distr of 1NN: G(x))

with witneses: we use the witnesses near the query to estimate the result of the query (produce distr of distances between a given query q and the witnesses: Fq(x), use this distr to produce the distr of 1NN: G(x))

say that their approach is very expensive, cannot scale

inspired by them , we propose our version of patella: distribution of 1NN of witnesses (G(x))

we will then show that this is not enough to give good results

we need to experimentally evaluate these approaches (with 100K series)








\subsection{1}

our approach1: 

we have random witnesses

when a query arrives, we compute the estimate of the query result based on the witnesses (eg, weighted average of their own NN)








\subsection{2}

our approach2: random witnesses

we have random witnesses
we also have some training queries, and we compute the estimate of the query result based on the witnesses, and the real query result, and then we compute the correlation between these two (we create a model that describes this relationship)

patella wants coverage because they are using a small number of witnesses, and for each witness they compute lots of information (distr of distances between witness and entire dataset)

above argument may be wrong... (since in any case, they use 3x the number of witnesses, and this is a random sample)










\subsection{3}

our approach3: correlation 1st bsf and 1nn

explain why correlation between 1st bsf and 1NN holds: indexes group similar series together, 1st bsf is computed by visiting the most promising/similar group of series

discuss kernel density estimation for the distrs

2-d kernel density estimation

note that this does not hold for UCR Suite, explain why not (1st bsf is not a good bsf)

we can give probabilistic quality guarantees

what can we say analytically?

can we give an analytic formula for the probabilistic guarantee?

note that our solution depends on the specific dataset

the distr we use can be used only for the specific dataset, and the specific size of the dataset (changing size means that the probs of finding a close neighbor may change)









\subsection{4}

our approach4 combined: correlation + witnesses

3-d kernel density estimation 

it seems that this does not help, because the estimates provided by approach3 (correlation 1bsf-1nn) are already much better than than approach2 random witnesses)

however, this may not be true for all datasets

if we have a dataset, where approach3 is not that good (deep1b?), then approach4 may help











\subsection{5}

our approach5 based on delayed bsf (wait till 100msec)

wait as much as you can while still being inside interactive response times

then do as above

this leads to much better approximations











\subsection{6}

approach6: knn case

how does our approach change here?

do we still talk about correlation (which exactly)?

can we use information from the first k-1 NN to better estimate the k-th NN?

density estimation: 
when a query arrives, get a probabilistic estimate of the density around that query; can use this for:

- adjusting the range of range queries

- information about the dataset (user understands what patterns exist, or not, in the dataset)

- a way to visualize the dataset (get random queries from our approach, present the ones that come from the dense parts of the dataset along with the density value)










\subsection{7}

approach7: overall bound from index sax representation, and individual segment bounds 

we will probably have a good estimate for the query result from approach3 (correlation 1bsf-1nn) that refers to entire query, and a less tight estimate for each segment of the query from the index sax representation

can we combine these two? can we use the approach3 estimate to improve the per segment estimate?










\subsection{visualization/hci}

\subsubsection{exploratory, no query execution} 

we observe that approach3 is in general better than approach2 (or approach1)

still, approach2 (or approach1) could be useful in the case, where we don't want to execute any query: approach2 (or approach1) can provide (almost) instantaneous estimates of the query results, without having to execute the query

useful when we have a large workload, and need a quick, rough first idea of how it behaves

useful for exploratory search




\subsubsection{per segment error}

approach7 can provide per segment estimates/bouds/errors

we can use those to visualize a per segment estimate of how we expect the results to look like (more fuzzy where we have loose estimates, more precise where we have tighter bounds)







==> evaluation_karima.tex <==
% !TEX root = main.tex

\section{Experimental Evaluation}
\label{sec:experiments}

%{\color{red}REVIEWER: The experiments do not cover the scalability issue well. Most of the places (including the technical presentation parts as well), only 1-NN is mentioned, although the problem is defined for k-NN.}

%{\bf ??? shall we change k-NN to NN? or add experiments with k-NN? ???} 

%\subsection{Setup}

%\vspace{5pt} 
\noindent{\bf Environment.}
All experiments were run on a Dell T630 rack server with two Intel Xeon E5-2643 v4 3.4Ghz CPUs, 512GB of RAM, and 3.6TB (2 x 1.8TB) HDD in RAID0. 
%All our search algorithms (ADS+ and DSTree) are single-core implementations. 

\vspace{5pt} 
\noindent{\bf Implementation.}  Our estimation methods were implemented in R. We use R's \emph{lm} function to carry our linear regression, the \emph{ks} library~\cite{ks} for multivariate kernel density estimation, and the \emph{quantreg} library~\cite{quantreg} for quantile regression. 
We use a grid of $200 \times 200$ points to approximate a 2D density distribution and a grid of $60 \times 180 \times 180$ points to approximate a 3D density distribution. 
%Denser grids did not result in measurable improvements in terms of precision. 
Source code and datasets are in~\cite{webpage}.

\vspace{5pt} 
\noindent{\bf Datasets.}
For the evaluation of the progressive similarity search techniques we used 1 synthetic and 3 real datasets from past studies~\cite{Zoumpatianos:2016,Echihabi:2018}, summarized in Table~\ref{tab:datasets}. 
All are \emph{100GB} in size with cardinalities and lengths reported in Table~\ref{tab:datasets}. 
Synthetic data series were generated as random walks (cumulative sums) of steps that follow a Gaussian distribution (0,1). 
This type of data has been extensively used in the past~\cite{conf/sigmod/Faloutsos1994,journal/kais/Camerra2014,conf/kdd/Zoumpatianos2015} and models the distribution of stock market prices~\cite{conf/sigmod/Faloutsos1994}. 
The IRIS seismic dataset~\cite{url/data/seismic} is a collection of seismic instrument recordings from several stations worldwide (100M series of length 256). 
The SALD neuroscience dataset~\cite{url/data/sald} contains MRI data (200M series of length 128). 
The image processing dataset, deep1B~\cite{url/data/deep1b}, contains vectors extracted from the last layers of a convolutional neural network (267M series of length 96). 

%\begin{table}
%	\centering
%	%\scriptsize
%	\caption{Experimental datasets for $k$-NN similarity search}
%	\begin{tabular}{ c|c|c|c} 
%		Name&Description&Cardinality&TS Length\\ \hline
%		%random & gaussian distrib. points on [0, 1] & 100 M & 256\\ \hline
%		synthetic & random walks & 100M & 256\\
%		seismic & seismic records & 100M & 256\\ 
%		SALD & MRI data & 200M & 128\\ 
%		deep1B & images & 267M & 96\\ 
%		%iEEG & 4 in 5 & 33 & 256\\ 
%	\end{tabular}
%	\vspace{-5pt}
%	\label{tab:datasets}
%\end{table}

\fanis{The above datasets are not annotated. In order to evaluate the progressive $k$-NN classification techniques, we use the datasets in Table~\ref{tab:datasets-classification}.}
% \textbf{Discuss the datasets: CBF~\cite{Saito:2000}, SITS~\cite{pelletier:2019}, and ImageNet~\cite{imagenet}}. 
\karima{The Cylinder-Bell-Funnel (CBF) dataset~\cite{Saito:2000} is a synthetic dataset consisting of data series belonging to one of three classes: cylinders, bells and funnels. Instances of each of class are generated randomly with Gaussian noise added, such that each series has  a fixed length of 128 but the onset and duration of each pattern varies randomly. An amplitude parameter is also used to control the difficulty of the dataset, where the smaller the amplitude, the less distinct the data series in different classes, thus the harder the classification task. We used the two amplitude values 1 and 3 to generate the CBF1 and CBF3 datasets respectively. {\bf ??? Themi, the original dataset used by Keogh~\cite{journal/dmkd/Keogh2003} had an amplitude of 6. This might raise some eyebrows. Shall we include an experiment with CBF6????}. 	}



\fanis{For ImageNet~\cite{imagenet}, image embeddings were generated using a pre-trained EfficientNetB1~\cite{EfficientNet} neural network. We applied a global average pooling to the last layers of the network to produce a single vector of 1280 real values per image. The dataset contains a total of 1361 distinct classes. For our experiments, we use the vectors of ImageNet's training images ($\approx 1.3$M images) as the series dataset and the vectors of its testing images (50K images, 1000 classes) to sample our queries. To also test our methods on a smaller number of classes, we used WordNet's~\cite{wordnet} hierarchical structure and grouped the original classes (``synsets") to 30 larger classes that correspond to the leaf nodes of the hierarchy used by Huang et al.~\cite{Huang2020}.}

\begin{table}
	\centering
	%\scriptsize
	\caption{Experimental datasets for $k$-NN classification {\bf ??? add text the describes these datasets, also the hardness factor of cbf ???} {\bf ??? Karima check the cbf sizes! ???}}
	\scalebox{0.88}{
	\begin{tabular}{c|c|c|c|c} 
		Name&Description&Cardinality&TS Length&Classes\\ \hline
		%random & gaussian distrib. points on [0, 1] & 100 M & 256\\ \hline
		CBF 1 & synthetic & 1M-10M & 128 & 3\\
		CBF 3 & synthetic & 1M-10M & 128 & 3\\ 
		SITS & satellite image pixels & 1M & 149 & 13 \\ 
		ImageNet & image embeddings & 1.3M & 1280 & 1361/30\\ 
	\end{tabular}
	\vspace{-5pt}
	\label{tab:datasets-classification}
	}
\end{table}



\vspace{5pt} 
\noindent{\bf Measures.} We use the following measures to assess the estimation quality of each method and compare their results:

\vspace{5pt} 
\noindent\emph{Coverage Probability:}  It measures the proportion of the time that the prediction intervals contain the true $1$-NN distance. 
If the confidence level of the intervals is $1-\theta$, the coverage probability should be close to $1-\theta$. A low coverage probability is problematic. In contrast, a coverage probability that is higher than its nominal value (i.e., its confidence level) is acceptable but can hurt the intervals' precision. In particular, a very wide interval that always includes the true $1$-NN distance ($100\%$ coverage) can be useless.

\vspace{5pt} 
\noindent\emph{Prediction Intervals Width:} It measures the size of prediction intervals that a method constructs. Tighter intervals are better.  However, this is only true if the coverage probability of the tighter intervals is close to or higher than their nominal confidence level. Note that for progressive distance estimates, we construct one-sided intervals. Their width is defined with respect to the upper distance bound $d_{Q,R}(t)$.

\vspace{5pt} 
\noindent\emph{Root-Mean-Squared Error (RMSE):}  It evaluates the quality of point (rather than interval) estimates by measuring the standard deviation of the true $1$-NN distance values from their expected (mean) values. 

%\vspace{5pt} 
To evaluate the performance of our stopping criteria, we further report on the following measures:

\vspace{5pt} 
\noindent\emph{Time Savings:} Given a load of queries and a stopping criterion, it measures the time saved as a percentage of the total time needed to complete the search without early stopping.

\vspace{5pt} 
\noindent\emph{Exact Answers:} It measures the number of exact answers as a percentage of the total number of queries. 
\fanis{For $k$-NN classification, we report on \emph{exact classes}, where we assess the percentage of queries for which the progressive class is the final one.}

\vspace{5pt} 
\fanis{
\noindent\emph{Accuracy Ratio:} We also measure the accuracy of $k$-NN classification of early stopping as a ratio of the accuracy of $k$-NN classification of exact search. 
}


\vspace{5pt} 
\noindent{\bf Validation Methodology.} To evaluate the different methods, we use a Monte Carlo cross-validation approach that consists of the following steps. 
For each dataset, we randomly draw two disjoint sets of data series $\mathcal{W}_{pool}$ and $\mathcal{T}_{pool}$ and pre-calculate all distances between the series of these two sets. 
The first set serves as a pool for drawing random sets of witnesses (if applicable), while the second set serves as a pool for randomly drawing training (if applicable) and testing queries. 
At each iteration, we draw $n_w$ witnesses ($n_w=50$, $100$, $200$, or $500$) and/or $n_r$ training queries ($n_r=50$, $100$, or $200$) from $\mathcal{W}_{pool}$ and $\mathcal{T}_{pool}$, respectively. 
We also draw $n_t=200$ testing queries from $\mathcal{T}_{pool}$ such that they do not overlap with the training queries. We train and test the evaluated methods and then repeat the same procedure $N = 100$ times, where each time, we draw a new set of witnesses, training, and testing queries. 
Thus, for each method and condition, our results are based on a total of $N \times n_t = 20K$ measurements. %100 \times 200 = 20000$ test measurements.

For all progressive methods, we test the accuracy of their estimates after the similarity search algorithm has visited $1$ ($2^0$), $4$ ($2^2$), $16$ ($2^4$),  $64$ ($2^6$), $256$ ($2^8$), and $1024$ ($2^{10}$) leaves. Figure~\ref{fig:leaves-distributions} shows the distributions of visited leaves for 100 random queries for all four datasets.  


\begin{figure}[tb]
\centering
\footnotesize
%\vspace{-5pt}
\includegraphics[width=0.95\linewidth]{leaves-distribution.pdf}
\vspace*{-2pt}
\caption{Distribution (over 100 queries) of the number of leaves visited (in $log_2$ scale) until finding the $1$-NN (light blue) and completing the search (yellow). The thick black lines represent medians.}
\label{fig:leaves-distributions}
%\vspace*{-0.6cm}
\end{figure}


\subsection{Results on Prediction Quality}
%\vspace{5pt} 
\noindent{\bf Previous Approaches.} We first evaluate the query-agnostic and query-sensitive approximation methods of Ciaccia et al.~\cite{Ciaccia:1999,Ciaccia:2000}. To assess how the two methods scale with and without sampling, we examine smaller datasets with cardinalities of up to 1M data series (up to 100K for the query-agnostic approach). Those datasets are derived from the initial datasets presented in Table~\ref{tab:datasets} through random sampling. Such smaller dataset sizes allow us to derive the full distribution of distances without sampling errors, while they are sufficient for demonstrating the behavior of the approximation methods as datasets grow. 

\begin{figure}[t]
\centering
\footnotesize
%\vspace{-1pt}
\includegraphics[width=1.\linewidth]{ciaccia-2.pdf}
\vspace{-10pt}
\caption{Coverage probabilities of query-agnostic (left) and query-sensitive (right) %approximation 
methods of Ciaccia et al.~\cite{Ciaccia:1999,Ciaccia:2000} for $95\%$ confidence level. We use 500 witnesses for the query-sensitive methods. We show best-case results (with the best $exp$: 3, 5, 12, or adaptive).}
\label{fig:results-ciaccia}
\vspace*{-2pt}
\end{figure}

Figure~\ref{fig:results-ciaccia} presents the coverage probabilities of the methods. The behavior of query-agnostic approximation is especially poor. Even when the full dataset is used to derive the distribution of distances, the coverage tends to drop below $10\%$ for larger datasets ($95\%$ confidence level). This demonstrates that the approximated distribution of $1$-NN distances completely fails to capture the real one. Figure~\ref{fig:ciaccia-distributions} compares the real to the approximated distributions for datasets of $100$K series. We observe that the method largely underestimates the $1$-NN distances for all four datasets. 

\begin{figure}[tb]
\centering
\footnotesize
%\vspace{-5pt}
\includegraphics[width=1.\linewidth]{ciaccia-distributions.pdf}
\vspace{-10pt}
\caption{Real distribution of $1$-NN distances and its query-agnostic approximation based on Ciaccia and Patella~\cite{Ciaccia:2000}. All datasets contain 100K series.}
\label{fig:ciaccia-distributions}
\vspace{-10pt}
\end{figure}

\begin{figure*}[t]
\centering
\footnotesize
%\vspace{-5pt}
\includegraphics[width=1.0\textwidth]{coverage-distance-estimates.pdf}
\vspace{-12pt}
\caption{Coverage probabilities of our estimation methods for $95\%$ and $99\%$ confidence levels. We show averages for the four datasets (synthetic, seismic, SALD, deep1B) and for 25, 50, 100, and 200 training queries.}
\label{fig:results-coverage}
\vspace{-4pt}
\end{figure*} 

\begin{figure}[t]
	\centering
	\footnotesize
	\hspace*{-5pt}
	\includegraphics[width=1.03\linewidth]{witnesses-width.pdf}
	\vspace{-12pt}
	\caption{The mean width of the $95\%$ PI for the witness-based query-sensitive method in relation to the number of witnesses and training queries.}
	\label{fig:results-witnesses}
\vspace{-10pt}
\end{figure}

Results for the query-sensitive method are better, but coverage is still below acceptable levels. Figure~\ref{fig:results-ciaccia} presents results for $n_w = 500$ witnesses. Note that our further tests have shown that larger numbers of witnesses result in no or very little improvement, while Ciacca et al.~\cite{Ciaccia:1999} had tested a maximum of $200$ witnesses. To weight distances (see Equation~\ref{eq:weights}), we tested the exponent values $exp = 3$, $5$, and $12$, where the first two were also tested by Ciacca et al.~\cite{Ciaccia:1999}, while we found that the third one gave better results for some datasets. We also tested the authors' adaptive technique.  Figure~\ref{fig:results-ciaccia} presents the best result for each dataset, most often given by the adaptive technique.

We observe that the GNAT method results in clearly higher coverage probabilities than the fully random method. This result is somehow surprising because Ciacca et al.~\cite{Ciaccia:1999} report that the GNAT method tends to become less accurate than the random method in high-dimensional spaces with more than eight dimensions. Even so, the coverage probability of the GNAT method is largely below its nominal level. In all cases, it tends to become less than $50\%$ as the cardinality of the datasets increases beyond 100K, while in some cases, it drops below $20\%$ (synthetic and seismic). 

For much larger datasets (e.g., 100M data series), we expect the accuracy of the above methods to become even worse. We conclude that they are not appropriate for our purposes, thus we do not study them further.

\vspace{4pt} 
\noindent{\bf Quality of Distance Estimates.} 
%We simplify our analysis by focusing on the ADS index (we examine %how our results generalize to  the DSTree index in the following subsection).  
We evaluate the coverage probability of $1$-NN distance estimation methods for confidence levels $95\%$ ($\theta=.05$) and $99\%$ ($\theta=.01$). Figure~\ref{fig:results-coverage} presents our results. The coverage of the \emph{Baseline} method reaches its nominal confidence level for $n_w = 200$ to $500$ witnesses. In contrast, the \emph{Query-Sensitive} method demonstrates a very good coverage even for small numbers of witnesses ($n_w = 50$) and training queries ($n_r = 25$). However, as Figure~\ref{fig:results-witnesses} shows, more witnesses increase the precision of prediction intervals, i.e., intervals become tighter while they still cover the same proportion of true $1$-NN distances. Larger numbers of training queries also help. 

The coverage probabilities of progressive estimates (Figure~\ref{fig:results-coverage}-Right) are best for the 2D kernel density approach, very close to their nominal levels. Linear regression leads to lower coverage, while the coverage of the 3D kernel density approach is more unstable. We observe that although the accuracy of the models drops in smaller training sets, coverage levels can still be considered as acceptable even if the number of training queries is as low as $n_r = 25$. 

%The coverage probabilities of \emph{individual linear} models are generally stable and very close to $95\%$ for $\theta = .05$. For $\theta = .01$, the coverage is around $97-98\%$, which suggests that the approach is relatively less accurate at high confidence levels. The 2D kernel density approach (\emph{individual kernel}) results in higher coverage for both confidence levels (expect for $2^{10} = 1024$ visited leaves). %with the exception of $2^{10} = 1024$ visited leaves, when coverage suddenly drops.
%Results for the \emph{common linear} model are less satisfying, especially for the very first stages of the progression algorithm ($<16$ visited leaves), where coverage is low. Coverage reaches very high levels ($>98\%$ for a $95\%$ confidence level) as more leaves are visited. As we explained earlier, this behavior may not be desirable since a very high coverage can be due to prediction intervals that are unnecessarily large. 
%The \emph{common kernel} density estimation method results in improved coverage levels. Coverage again tends to further increase as the number of visited leaves grows. 

Figure~\ref{fig:results-comparison} compares the quality of initial and early (i.e., based on first approximate answer) estimates provided by different techniques: (i) Baseline, (ii) Query-Sensitive method, (iii) 2D kernel density estimate for iSAX2+, and (iii) 2D kernel density estimate for DSTree.
%two methods of initial estimates (Baseline and Query-Sensitive) against estimation based on the 1st approximate answer of the ADS index (see Figure~\ref{fig:bsf-fit}). For this latter method, we construct individual linear models, where \emph{Leaves Visited} $= 1$.
For all comparisons, we set $n_w = 500$ and $n_r = 100$. For these parameters, the coverage probability of all methods is close to $95\%$. 
We evaluate the width of their $95\%$ prediction intervals and RMSE. We observe similar trends for both measures, where the query-sensitive method outperforms the baseline. 
We also observe that estimation based on the first approximate answer (at the first leaf) leads to radical improvements for all datasets. 
Overall, the DSTree index gives better estimates than iSAX2+.  

\begin{figure}[tb]
\centering
\footnotesize
%\hspace*{-7pt}
\includegraphics[width=1.0\linewidth]{comparison-violin.pdf}
\vspace{-12pt}
\caption{Violin plots showing the distribution of the width of $95\%$ prediction intervals (top) and the distribution of the RMSE of expected $1$-NN distances (bottom). We use $n_w = 500$ (baseline and query-sensitive method) and $n_r = 100$ (query-sensitive method and 2D kernel model for the 1st approximate answer).}
\label{fig:results-comparison}
%\vspace{-15pt}
\end{figure}

As shown in Figure~\ref{fig:ads-progressive}, progressive answers lead to further improvements. The RMSE is very similar for all three estimation methods, which means that their point estimates are equally good. Linear regression results in the narrowest intervals, which explains the lower coverage probability of this method. Overall, 2D kernel density estimation provides the best balance between coverage and interval width. 


%Both kernel density estimation methods provide a good balance between coverage and size but produce wider intervals than individual linear models.  

%Overall, we can conclude that all models are equally good at providing point distance estimates. Yet, using individual models results in more precise intervals, as the approach allows for a better control of coverage levels. 

\begin{figure}[t]
\centering
\footnotesize
\hspace*{-7pt}
\includegraphics[width=1.05\linewidth]{width-rmse.pdf}
\vspace{-10pt}
\caption{Progressive models: Mean width of $95\%$ prediction intervals of $1$-NN distance estimates and RMSE. %We also show the relative error as a percentage of the $1$-NN distance. 
Results are based on $n_r=100$ training queries.}
\label{fig:ads-progressive}
%\vspace{-10pt}
\end{figure}

%\vspace{5pt} 
%\noindent{\bf DSTree Index.} We observe similar patterns with the DSTree index~\cite{Wang:2013:DDS}. Figure~\ref{fig:dstree-progressive} summarizes our experimental results for this algorithm. 
%All methods result in similar RMSE scores, but provide a different balance between coverage and interval width. The individual linear models present a less variable coverage probability that is very close to $95\%$ and produce tigher intervals. Prediction intervals constructed with a common linear model are again the worst with very variable coverage levels.  If we compare Figure~\ref{fig:ads-progressive} and Figure~\ref{fig:dstree-progressive}, we further observe that the DSTree index produces more precise estimates than the ADS index and very low errors at the very first leaves. 
%\fanis{Say something more about these two algorithms.}

%\begin{figure}[t]
%\centering
%\footnotesize
%%\vspace{-5pt}
%\includegraphics[width=1.\linewidth]{DSTree-results.pdf}
%\vspace{-15pt}
%\caption{Coverage probability ($95\%$ confidence level), mean width of $95\%$ prediction intervals, and RSME of our temporal models using the DSTree index. All results are based on $n_r=100$ training queries.}
%\label{fig:dstree-progressive}
%\vspace{-10pt}
%\end{figure}

%\begin{figure}[t]
%\centering
%\footnotesize
%%\vspace{-5pt}
%\includegraphics[width=1.\linewidth]{DSTree-all.pdf}
%%\vspace{-15pt}
%\caption{Coverage probability ($95\%$ confidence level), mean width of prediction intervals, and RSME of progressive models for the DSTree index. All results are based on $n_r=100$ training queries.}
%\label{fig:dstree-progressive}
%%\vspace{-10pt}
%\end{figure}


%\vspace{5pt} 
%\noindent{\bf Subsequences.} 
%We can apply the same approach to provide distance estimates for the subsequences of the $1$-NN (see Section~\ref{sec:progressive}).
%Table~\ref{tab:subsequences} reports the coverage probability of $95\%$ prediction intervals predicting the partial distance of $16$ individual segments of the $1$-NN. Results are based on the fist approximate answer (\emph{Visited Leaves} $= 1$) of iSAX2+ and $n_r=200$ training queries when using linear regression. Average coverage levels are slightly lower than nominal levels ($\simeq 94\%$ on average) but still acceptable. 
%
%\begin{table}[tb]
%	\centering
%	\small
%	\caption{Coverage Probabilities for Subsequences}
%	\begin{tabular}{ c||c c c} 
%		Dataset &Full Series & Subseq. (mean) & Subseq. (min)\\ \hline
%		synthetic & 95.2\% & 94.6\% & 94.1\%\\
%		seismic & 95.9\% & 94.0\% & 93.5\%\\ 
%		SALD & 94.4\% & 92.8\% & 92.1\%\\ 
%		deep1B & 95.0\% & 94.7\% & 94.3\%\\ \hline
%		Overall & 95.1\% & 94.0\% & 93.7\%
%	\end{tabular}
%	\begin{tablenotes}
%      \small
%      \item \textbf{Note:} We report coverage probabilities ($95\%$ confidence level) for 16 data series subsequences when estimating the sub-distance of the 1-NN from the 1st approximate answer of iSAX2+. All results are based on $n_r=200$ training queries.
%    \end{tablenotes}
%	\label{tab:subsequences}
%\end{table}
%
%A key question is whether distance estimation on individual subsequences helps reduce uncertainty. Figure~\ref{fig:distance-subsequences} shows the distribution of the lower and upper bounds of the $95\%$ prediction intervals constructed for both full series and their subsequences. We observe that the approach allows us to derive tighter bounds for subsequences. In particular, the upper bounds are greatly lower than the ones determined by the intervals that we construct for the full series distances. Likewise, for several queries, lower bounds are considerably greater than zero, which is the hard lower bound that we get in the absence of other information.  
%
%\begin{figure}[tb]
%\centering
%\footnotesize
%\includegraphics[width=1.\linewidth]{subs-bounds.pdf}
%\caption{Violin plots showing the distributions of low (blue/left) and upper (yellow/right) bounds of the $95\%$ prediction intervals (1st approximate answer of iSAX2+) of the distance for the full 1-NN and for its 16 subsequences. The thick black lines show medians. Training is based on $n_r=200$ queries.}
%\label{fig:distance-subsequences}
%\end{figure}
%
%

\begin{figure}[t]
	\centering
	\footnotesize
	\includegraphics[width=1.0\linewidth]{sequential-exact.pdf}
	\vspace{-12pt}
	\caption{(a) Effect of 3 and 5 sequential tests on the coverage of $95\%$ and $99\%$ prediction intervals. We use 2D kernels with $n_r = 100$. (b) Coverage of exact answers for time upper bounds ($95\%$ and $99\%$ conf. levels).}
	\label{fig:results-sequential}
\end{figure} 

\vspace{4pt} 
\noindent{\bf Sequential Tests.} 
We assess how multiple sequential tests (refer to Section~\ref{sec:progressive}) affect the coverage probability of $1$-NN distance prediction intervals. 
We focus on 2D kernel density estimation ($n_r = 100$), which gives the best coverage (see Figure~\ref{fig:results-coverage}). 
We examine the effect of (i) three sequential tests when visiting 1, 512, and 1024 leaves, and (ii) five sequential tests when visiting 1, 256, 512, 768, and 1014 leaves. 
We count an error if at least one of the three, or five progressive prediction intervals do not include the true $1$-NN distance. 

%Figure~\ref{fig:results-sequential}(a) summarizes our results. 
As results for DSTree and iSAX2+ were very close, we report on their means (see Figure~\ref{fig:results-sequential}(a)). 
The coverage of $95\%$ prediction intervals drops from over $95\%$ to about $90\%$ for five tests (higher for seismic and lower for deep1B). 
Likewise, the coverage of their $99\%$ prediction intervals drops to around $95\%$. 
%In contrast, individual linear models are more sensitive to sequential testing and result in lower coverage levels. In particular, the coverage of their $99\%$ prediction intervals becomes clearly lower than $95\%$ for all but one dataset. When sequential testing is an issue, we recommend using either of the two kernel methods, as their coverage level is more stable across datasets. 
%Adjusting the confidence level to account for multiple sequential comparisons is still an open question. 
These results provide rules of thumb on how to correct for multiple sequential tests, e.g., use a $95\%$ level in order to guarantee a $90\%$ coverage in $5$ sequential tests. 
Notice, however, that such rules may depend on the estimation method and the time steps at which comparisons are made. 
An in-depth study of this topic is part of our future work.

\vspace{4pt} 
\noindent{\bf Time Bounds for Exact Answers.}  We are also interested in the quality of time guarantees for exact answers (refer to Section~\ref{sec:exact}). We evaluate the coverage of our time bounds for $50$, $100$, and $200$ training queries for confidence levels $95\%$ ($\phi = .05$) and $99\%$ ($\phi = .01$). 
Figure~\ref{fig:results-sequential}(b) summarizes our results. 
We observe that coverage is good for training samples of $n_r \geq 100$, but drops for $n_r = 50$. %It is well-known that quantile regression is not accurate in small samples, but a workaround is to use more conservative bounds through bootstrapping methods.

\begin{figure}[tb]
	\centering
	\footnotesize
	%\vspace{-5pt}
	\includegraphics[width=1.0\linewidth]{stopping-error-2.pdf}
	\vspace{-12pt}
	\caption{Evaluation of the stopping criterion that bounds the distance error ($\epsilon_Q < \epsilon$). We use $95\%$ prediction intervals ($\theta = .05$) and $n_r=100$ training queries.}
	\label{fig:stopping-criteria-epsilon}
	\vspace{-5pt}
\end{figure} 

\begin{figure*}[tb]
	\centering
	\footnotesize
	%\vspace{-5pt}
	\includegraphics[width=1.0\textwidth]{stopping-phi-results-2.pdf}
	\vspace{-10pt}
	\caption{Evaluation of stopping criteria that bound ($\phi$) the probability/ratio of non-exact answers. We measure their ratio of exact answers and their time savings ($\%$). For all conditions, we use $n_r=100$ training queries.}
	\label{fig:stopping-criteria-phi}
%	\vspace{-5pt}
\end{figure*} 

\begin{figure*}[tb]
	\centering
	\footnotesize
	\includegraphics[width=1.0\textwidth]{deep-workload-2.pdf}
	\vspace{-10pt}
	\caption{Performance of our stopping criteria for a real workload of 600 queries (deep1B dataset and DSTree). We draw $n_r = 50$ or $100$ random queries for training. We then apply a criterion to the remaining queries. Answers with $\epsilon_Q  < \epsilon$ and exact ones ($\%$) are measured for those ``testing'' queries. (We report means over 100 repetitions.)}
	\label{fig:deep}
\end{figure*} 


%\vspace{5pt} 

\subsection{Results on Time Savings}
We compare our stopping criteria (see Section~\ref{sec:stopping}) and assess the time savings they offer. 
Figure~\ref{fig:stopping-criteria-epsilon} shows results for our first criterion that bounds the distance error. 
We consider $16$ discrete and uniform moments $t_i$, where $t_{16}$ is chosen to be equal to the maximum time it takes to find an exact answer in the training sample. 
For each $t_i$, we train an individual 2D kernel density and use $95\%$ prediction intervals ($\theta = .05$) for estimation.   
The coverage (ratio of queries for which $\epsilon_Q  < \epsilon$) exceeds its nominal level ($95\%$) for all datasets, which suggests that results might be conservative. The reason is that stopping could only occur at certain moments. For higher granularity, one can use a larger number of discrete moments. The ratio of exact answers is close to $95\%$ for $\epsilon = .01$ but becomes unstable for $\epsilon = .05$, dropping to as low as $70\%$ for the seismic dataset. 
On the other hand, this results in considerable time savings, especially for DSTree: higher than $90\%$ for the synthetic, SALD, and deep1B datasets.

Figure~\ref{fig:stopping-criteria-phi} compares the two stopping criteria 
%(time bound and probability) 
that control the ratio of exact answers. 
For the probability criterion, we consider again $16$ discrete moments to stop the search, as above. 
The time-bound criterion results in mean exact answer ratios that are very close to nominal levels, while the probability criterion is rather conservative. 
However, the time gains of the two techniques are comparable. 
For iSAX2+, the probability criterion achieves both a higher accuracy and higher time savings than the probability criterion. 
In contrast, both criteria lead to similar time savings for DSTree, reducing query %answering 
times by up to 95\%.

%The $\phi$ parameter of the exact-answers criterion controls the ratio of exact answers with high accuracy (also see Figure~\ref{fig:results-sequential}b). This good behavior is consistent across all datasets and index methods. For the distance-error criterion, the ratio of exact answers is extremely variable. It is close to $95\%$ for $\epsilon = .01$ but becomes unstable for $\epsilon = .05$, dropping to as low as $70\%$ for the seismic dataset. Nevertheless, the requirement for exact answers is rather strict; users may simply want to bound their $1$-NN distance error. 



%As shown in Figure~\ref{fig:stopping-criteria}-Right, both stopping criteria result in significant performance gains. Cost cuts are especially pronounced for the DSTree index -- the stopping time drops below $.1$ for the three datasets (synthetic, SALD, and deep1B). As expected, stricter $\phi$ and $\epsilon$ thresholds lead to higher costs. Direct comparisons between the two stopping criteria are difficult, as the two methods have different parameters. }

%A major strength of the 

%However, it is interesting to compare the results of $\phi = .05$ and $\epsilon = .01$ since both result in similar rates of exact answers ($\approx95\%$).

\vspace{4pt} 
\noindent{\bf Training Costs vs. Gains.} Training linear models with $100$ queries is instantaneous, while learning $16-20$ density functions with 2D kernel density estimation takes no more than 4-6 seconds on a regular laptop. 
Of course, our approach requires the full execution of the training queries. 
For a detailed analysis of the costs of exact similarity search with iSAX2+ and DSTree, we refer the reader to the results of Echihabi et al.~\cite{Echihabi:2018}. Depending on the size and type of the dataset, processing $100$ queries can take some dozens of minutes ($50$ GB datasets), or several hours ($250$ GB datasets). 
Nevertheless, the higher this initial training cost, the higher the benefit is when users later execute their queries. 

Figure~\ref{fig:deep} shows the results for the first 600 queries extracted from a real query workload that comes with the deep1B dataset. 
(Experiment conducted on a server with two Intel Xeon E5-2650 v4 2.2GHz CPUs, 75GB of RAM.)
Results are based on 100 repetitions; each time we draw at random 50, or 100 queries for training. 
We then apply our stopping criteria to accelerate the remaining queries.

The results show that our approach leads to significant performance improvements, while coverage (exact answers, or answers with $\epsilon_Q  < \epsilon$) is very close to, or higher than the nominal levels, even with training sizes of only $50$ queries.
For example, this workload of 600 queries would normally take 76 hours to execute with the DSTree index, but we can execute it in less than 20 hours (probability criterion; including training time), while achieving an average coverage of more than $95\%$ exact answers. 
Finally, we note that, as the trends in the graphs show, the  time savings and speedup offered by our progressive similarity search techniques will increase as the size of the query workload increases. 
%using our 2D kernel model, we can execute it 7x faster while guaranteeing that 95\% of the answers will be the exact ones.



%To better assess training costs, we emphasize the following two points. First, users may have no prior idea about their queries and derive them as they interact with their data. In this case, training can happen offline on a random query sample. Then, users can benefit from progressive search when they are in front of their screen. Training data are negligible in size and can be easily shared and reused. Second, such training does not necessarily introduce additional costs, as unlike indexing, it does not constrain normal query execution. Take the scenario where a user needs to process a workload of $1000$ queries. Query execution can start with a random sample of $50-100$ of these queries with no extra cost. These queries can then be used as a training set, and execute the rest of the $900-950$ queries with huge time gains (see Figure~\ref{fig:stopping-criteria}).


%unlike indexing, such training does not constraint the 

%Finally, we evaluate the time that it takes to process a random set of training queries, required by our methods. Figure~\ref{fig:training-time} presents results for ADS and DSTree for $n_r$=$100$. 
%Our results 
%corroborate the results of Echihabi et al.~\cite{Echihabi:2018}, showing 
%show that DSTree results in faster query completion, but for a higher indexing cost. 
%Even though we report the index creation cost, we note that we could train a model on an existing index, paying only the query answering cost for the $n_r$ queries. 
%Overall, we can train our models in $\sim$50min for 100GB datasets (average DSTree query answering performance), or $\sim$2hours for 250GB datasets, and then use these models to support large numbers of progressive queries by multiple users with very high coverage (see Figures~\ref{fig:results-coverage} and~\ref{fig:dstree-progressive}).

%We note that training the best competitor, the distance distribution of the GNAT query-sensitive approach~\cite{Ciaccia:1999} with $500$ witnesses (equivalent to computing the distances of \emph{all} $500$ witnesses to \emph{every single} series in the dataset) requires $\sim$2hours for 100GB and $\sim$4hours for 250GB. 
%Yet, the coverage of GNAT is less than half the coverage that our methods achieve (see Figure~\ref{fig:results-ciaccia}), and unacceptably low for our needs. 

%\begin{figure}[t]
%\centering
%\footnotesize
%%\vspace{-5pt}
%\includegraphics[width=1.\linewidth]{training-time.pdf}
%%\vspace{-15pt}
%\caption{Time to process 100 training queries, varying dataset size: ADS (top), DSTree (bottom).} %for datasets of 25 to 250 GB (up to 100 GB for the seismic dataset).}
%\label{fig:training-time}
%%\vspace{-10pt}
%\end{figure}

\fanis{
\subsection{Results for $k$-NN Similarity Search}
We evaluate how well our approach generalizes to $k$-NN similarity search. We follow the same experimental method and use the same four datasets but focus on the performance of our stopping criteria. Figure~\ref{fig:knn-search} summarizes our evaluation results. We first show the average savings in time if stopping was optimally performed by an oracle that knows when a $k$-NN is found (Figure~\ref{fig:knn-search}a). We observe that optimal time savings deteriorate as $k$ increases. This is especially the case for the seismic dataset, e.g., savings reduce from $87\%$ ($k=1$) to $45\%$ ($k=100$) when iSAX2+ is used.

For the distance-error criterion, we report results for $\theta = .05$ and $\epsilon = .05$ (Figure~\ref{fig:knn-search}b), where we now control and evaluate the relative family-wise distance error $\epsilon^f_Q$ (see Equation~\ref{eq:family-error}). For iSAX2+, time savings are stable and high (above $70\%$) across the full range of $k$ values. This comes at the cost of a decreasing ratio of exact answers. For DSTree, time savings drop for $k = 5$ but stay constant after, with the exception of the seismic dataset, where time savings stay constant but the ratio of exact answers significantly drops. Overall, the distance-error stopping criterion provides a way for quickly finding low-error answers, which may not be exact. 

Figure~\ref{fig:knn-search}b presents results for the time-bound and probability criteria. The probability criterion has a better ratio of exact answers but time savings for both criteria are very similar and drop as $k$ increases. Time savings become as low as $10\%$ for the seismic dataset and $k \geq 50$ (iSAX2+).  
}

\begin{figure*}[tb]
	\centering
	\footnotesize
	%\vspace{-5pt}
	\includegraphics[width=0.99\textwidth]{vldb-kNN-stopping.pdf}
	\vspace{-2pt}
	\caption{\fanis{Evaluation of our stopping criteria for $k$-NN similarity search ($n_r=100$ training queries). (a) Optimal time savings if an oracle stopped the search as soon as the exact $k$-NN was found. (b) Results for the distance-error criterion, where $\epsilon^f_Q$ refers to the maximum, i.e., family-wise, distance error among all $k$ nearest neighbors. (c) Results for the time-bound criterion and the probability criterion.}}
	\label{fig:knn-search}
	\vspace{-5pt}
\end{figure*} 

\fanis{
\subsection{Results for \fanis{$k$-NN Classification}}
\label{sec:experiments-classification}

\begin{figure*}[tb]
	\centering
	\footnotesize
	%\vspace{-5pt}
	\includegraphics[width=0.99\textwidth]{vldb-kNN-Classification.pdf}
	\vspace{-2pt}
	\caption{\fanis{Results for $k$-NN classification. (a) Evolution of answers to $10$-NN classification queries. We average a random sample of 1000 queries per dataset. For each step, we show the percentage of queries for which the current $10$-NN is exact (top) and the percentage of queries for which the current class is exact (bottom). (b) Results for our conservative stopping criterion that assesses the probability that the current $k$-NN is exact. (c) Results for our class-level criterion that assesses the probability that the current class is exact. We use $n_r = 100$ training queries. {\bf ??? Karima what cbf sizes are we using in each experiment? ???}}}
	\label{fig:knn-classification}
	\vspace{-5pt}
\end{figure*} 

}


\begin{figure}[t]
	\centering
	\footnotesize
	\includegraphics[width=1.0\linewidth]{cardinality-classification.pdf}
	\vspace{-12pt}
	\caption{\fanis{Coverage and time savings ($\phi_c = .05$) for different sizes of the CBF1 dataset when $k=10$. We present results for Euclidean Distance and DTW. We use $n_r = 100$ training queries}.}
	\label{fig:classification-cardinality}
\end{figure} 




==> new-approach.tex <==
\section{Approach-New}
\label{sec:approach}

\subsection{Possible Approach}

The best choice of k and weights depends upon the data, so we may take k and weights as input from the user. A common weighting scheme consists in giving each neighbor a weight of 1/d, where d is the distance to the neighbor. 
We may use the confidence probability of the prediction class as the stopping criterion. Prediction class is the class with the highest "score" Stop execution when the probability that prediction class is same as the class that would be reported by an exact Knn classifier is above some threshold. 
Possible algorithm to calculate this probability: Let's say we have \textbf{c} number of classes, \textbf{m} "exact" answers for the first \textbf{m} nearest neighbors, and \textbf{k-m} BSFs (0$\leq$m$\leq$k) at any instant. Initially m=0, finally m=k (if no early stopping). We also have \textbf{k-m} confidence probabilities for each BSF and a sequence of weights as a parameter for the k neighbors. We have a class mapping \textbf{C(.):} set of time series $\xrightarrow{}$ set of classes. For each class, we have two fields, namely ExactContribution and BSFContribution, which are 0 initially. $\alpha,W,B$ are 3 parameters to adjust. This algorithm could be run at discrete time intervals. Rough algorithm is shown in Algorithm~\ref{alg:Knn}.

{\bf ??? 1. can we write the same code by removing the "exact" special case? just treat these cases as answers with prob=1 ???}

{\bf ??? 2. prob of current bsf can also be a *range* (eg, [0.6-0.7]) ???}

{\bf ??? 3. weight can be a function of the distance to that neighbor ???}

{\bf ??? 4. the input probs for the BSFs can be prob distributions for the final distance ???}

{\bf ??? 5. in our algorithm, we need to compute the *prob that the current majority class will be the final majority class*; in order to do that we need the estimate and prob of the final NN distance (simply having the prob that the current NN is the final one, is probably not enough) ???}

{\bf ??? 6. the ideas in vfdt ???}

{\bf ??? 7. motivation: petitjean remote sensing classification, facebook images faiss paper, extreme classification(?): we have to argue that it is ok to spend pre-processing time (index building, etc), rather than use more complex classifier that would then classify very fast ???}

{\bf ??? 8. see standard Knn implementation: https://scikit-learn.org/stable/modules/generated/sklearn.neighbors.KNeighborsClassifier.html ???}

{\bf ??? meeting minutes May22 ???}
It is possible that we have an intermediate kNN answerset with low confidence that it is correct, but at the same time high confidence that the classes are correct! 
This may happen if the classes are well separated (so we know the correct class but not the exact NNs)
So training and using a model on the kNN classification task per se (instead of using the sigmod20 model) may result in higher time savings.
Do we need to take into account in this model the prior distribution of classes (prob of each class label)?

Use cbf as the default dataset to test our framework under different situations (vary dataset size, number of classes, similarity between classes, prob of each class)\\

\noindent{\bf Lower bound DTW for APCA:}\\
Assume APCA representation has $M$ segments\\
$r_i$ $\xrightarrow{}$ the right end time instant for segment $i$ $(1 \leq i \leq M)$

\[
\hat{U_i} = max(U_{r_{i-1}+1},\ U_{r_{i-1}+2},\ \dots\ ,\ U_{r_{i}})
\]

\[
\hat{L_i} = min(L_{r_{i-1}+1},\ L_{r_{i-1}+2},\ \dots\ ,\ L_{r_{i}})
\]

\[
LB\_APCA(Q,\Bar{C}) = \sqrt{\sum_{i=1}^{M}(r_i-r_{i-1})\begin{cases}
  (\bar{c_i}-\hat{U_i})^2&\text{if  }\bar{c_i}>\hat{U_i}\\    
  (\hat{L_i}-\bar{c_i})^2&\text{if  }\bar{c_i}<\hat{L_i}\\
  0 &otherwise
\end{cases}}
\]

\[
LB\_APCA(Q,\Bar{C}) \leq LB\_Keogh(Q,C)
\]

\noindent{Assume an EAPCA node contains a set of time series $Y_1,\dots,Y_l$ with synopsis $\textbf{Z} = (z_1,z_2,\dots,z_M)$ where $z_i = (\mu_i^{min},\mu_i^{max})$ where $\mu_i^{min} = min(\mu_i^{Y_1},\dots,\mu_i^{Y_l})$ and $\mu_i^{max} = max(\mu_i^{Y_1},\dots,\mu_i^{Y_l})$. Then, $MINDIST(Q,Z)$

}

\[
 = \sqrt{\sum_{i=1}^{M}(r_i-r_{i-1})\begin{cases}
  (\mu_i^{min}-\hat{U_i})^2&\text{if  }\mu_i^{min}>\hat{U_i}\\    
  (\hat{L_i}-\mu_i^{max})^2&\text{if  }\mu_i^{max}<\hat{L_i}\\
  0 &otherwise
\end{cases}}
\]

\[
 MINDIST(Q,Z) \leq LB\_APCA(Q,\Bar{Y_j})\ \forall\ 1\leq j \leq l
\]


\begin{algorithm}[tb]
	{
		\SetAlgoLined
% 		\KwIn{\textbf{Exact Answers} $e_1,..,e_m$,\textbf{BSFs} $b_{m+1},..,b_k$, \textbf{BSF confidence prbabilities} $p_{m+1},..,p_k$,  \textbf{Class map} $C(.)$}
        \KwIn{\textbf{Progressive Answers} $b_{1},b_2,...,b_k$, \textbf{Confidence Probabilities} $p_1,p_2,...,p_k$, \textbf{Class map} $C(.)$}
		\KwOut{$ClassConfidence$}
		
		\textbf{float} $Scores[]$, $ProbDist[]$ \tcp*{\footnotesize{initialize}}
% 		\For{$cl$ in $classes$ }
% 		{   
% 		    $cl.ExactContribution$\leftarrow$0$\\
% 		    $cl.BSFContribution$\leftarrow$0$\\
% 		}
		
% 		\For{$i$ $\leftarrow$  $1$ \emph{\KwTo} $m$}
% 		{   
% 		    $C(e_i).ExactContribution$ $+=$ $1$\\
%         }
        
        \For{$i$ $\leftarrow$  $1$ \emph{\KwTo} $k$}
		{   
		    $Scores[C(b_i)]$ $+=$ $p_i$\\
		    \For{$class$ $\neq$ $C(b_i)$ in $classes$}
    		{   
    		    $Scores[class]$ $+=$ $(1-p_i)/(c-1)$\\
    		}
        }
		
% 		\textbf{class} $Max1$ \tcp*{\footnotesize{class with max $ExactContribution$}}\\
% 		\textbf{class} $Max2$ \tcp*{\footnotesize{class with second max $ExactContribution$}}\\
		
% 		\uIf{$Max1$ $>$ $Max2$ + $k-m$}
% 		{
% 		    $ClassConfidence$ \leftarrow $1$\\
% 		}
        $CheckForTermination()$\\
        $Normalize(Scores)$\\
        
       $ProbDist_i  = \frac{exp(Scores[i])}{\sum_{j}^{ }exp(Scores[j])}$
	    
% 	    \For{$i$ $\leftarrow$  $1$ \emph{\KwTo} $c$}
% 		{   
% 		    $Score$[i] \leftarrow \alpha*$class_i.ExactContribution$ + $class_i.BSFContribution$\\
% 		    // \alpha \geq $1 to enhance effect of exact answers$\\
%         }
%         \For{$i$ $\leftarrow$  $1$ \emph{\KwTo} $c$}
% 		{   
% 		    $Score$[i] \leftarrow W*$Score$[i] + B\\
% 		    // Apply Weight and bias
%         }
        
%         //get probability distribution by applying softmax function on scores to enhance the difference between scores\\
        
        $ClassConfidence \leftarrow max(ProbDist)$\\
	    
		
		\Return $ClassConfidence$\\
	}
	\caption{Rough Algorithm (Uniform Weights)}
	\label{alg:Knn}
\end{algorithm}



% EXAMPLE PSEUDOCODE %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%Our algorithm is shown in Algorithm~\ref{alg:simpleKnn}.
% Pay attention to Line~\ref{simpleKnn:TrueCond}, and then we return the answer in Line~\ref{simpleKnn:return}.
% \begin{algorithm}[tb]
% 	{
% 		\SetAlgoLined
% 		\KwIn{\textbf{QuerySeries} $QDS$,\textbf{QuerySeries} $QDS_g$, \textbf{query iSAX} $isax$, \textbf{iSAX summarizations} $SAX$[],  \textbf{Index} $index$,\textbf{Bool} $Cmap$[],\textbf{Bool} $Cmap_g$[]}
% 		\KwOut{$realDistance$}
		
% 		\textbf{float} $BSF$ \tcp*{\footnotesize{initialize}}
		
% 		\For{$i$ $\leftarrow$  $0$ \emph{\KwTo}$ Datasize$\label{LBgpu:loop}}
% 		{
% 			float distance=0;
% 			\For{$j$ $\leftarrow$  $0$ \emph{\KwTo} paasegmentsize -1}
% 			{
% 				\textbf{float} breakpointupper=breakpointdictionaly[SAX[i*paasegmentsize+j]+1]\;\label{LBgpu:bkpu} 
% 				\textbf{float} breakpointlower=breakpointdictionaly[SAX[i*paasegmentsize+j]]\;\label{LBgpu:bkpl} 
% 				\uIf{$QDS_g[j]<breakpointlower$}
% 				{	
% 					$distance+=(breakpointlower-(QDS_g[j])^2$\;\tcp*[f]{ Perform an approximate search}\\
% 				}
% 				\ElseIf{$QDS_g[j]>breakpointuper$}
% 				{
% 					$distance+=(breakpointuper-(QDS_g[j])^2$\;
% 				}
				

% 			}
% 			\uIf{distance$<$ BSF}
% 			{
% 				$Cmap_g$[$i$]=True \label{simpleKnn:TrueCond} \tcp*{\footnotesize{has <= $2^w$ children}}
% 			}
% 			\Else
% 			{
% 			$Cmap_g$[$i$]=False\;
% 			}
% 		}
% 		\Return ($BSF$)\;\label{simpleKnn:return}
% 	}
% 	\caption{LowerBound\_GPU}
% 	\label{alg:simpleKnn}
% \end{algorithm}
%
% EXAMPLE PSEUDOCODE %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%




==> new-conclusions.tex <==
\section{Conclusions-New}
\label{sec:conclusion}

In this work, we argued for the usefulness (and need) of progressive answering of similarity search queries on very large time series data. 
We explored the use of the proposed solutions 
for speeding up complex analysis algorithms, i.e., $k$-NN classifiers and discord discovery, by enabling them to automatically decide when to stop a similarity search query early, without sacrificing the accuracy of the overall process.

Our experimental results with XXXXXXXXXXXXXXX datasets, demonstrate XXXXXXXXXXXXXXXXX







==> new-evaluation.tex <==
% !TEX root = main.tex

\section{Experimental Evaluation-New}
\label{sec:experiments}

%\vspace{5pt} 
\noindent{\bf Environment.}
All experiments were run on a Dell T630 rack server with two Intel Xeon E5-2643 v4 3.4Ghz CPUs, 512GB of RAM, and 3.6TB (2 x 1.8TB) HDD in RAID0. 
%All our search algorithms (ADS+ and DSTree) are single-core implementations. 

\vspace{5pt} 
\noindent{\bf Implementation.}  Our estimation methods were implemented in R. We use R's \emph{lm} function to carry our linear regression, the \emph{ks} library~\cite{ks} for multivariate kernel density estimation, and the \emph{quantreg} library~\cite{quantreg} for quantile regression. 
We use a grid of $200 \times 200$ points to approximate a 2D density distribution and a grid of $60 \times 180 \times 180$ points to approximate a 3D density distribution. 
Denser grids did not result in measurable improvements in terms of precision. 
Source code and datasets are in~\cite{webpage}.

\vspace{5pt} 
\noindent{\bf Datasets.}
We used 1 synthetic and 3 real datasets from past studies~\cite{Zoumpatianos:2016,Echihabi:2018}. 
All are \emph{100GB} in size with cardinalities and lengths reported in Table~\ref{tab:datasets}. 
Synthetic data series were generated as random walks (cumulative sums) of steps that follow a Gaussian distribution (0,1). 
This type of data has been extensively used in the past~\cite{conf/sigmod/Faloutsos1994,journal/kais/Camerra2014,conf/kdd/Zoumpatianos2015} and models the distribution of stock market prices~\cite{conf/sigmod/Faloutsos1994}. 
The IRIS seismic dataset~\cite{url/data/seismic} is a collection of seismic instrument recordings from several stations worldwide (100M series of length 256). 
The SALD neuroscience dataset~\cite{url/data/sald} contains MRI data (200M series of length 128). 
The image processing dataset, deep1B~\cite{url/data/deep1b}, contains vectors extracted from the last layers of a convolutional neural network (267M series of length 96). 

\begin{table}
	\centering
	%\scriptsize
	\begin{tabular}{ c|c|c|c} 
		Name&Description&Cardinality&TS Length\\ \hline
		%random & gaussian distrib. points on [0, 1] & 100 M & 256\\ \hline
		synthetic & random walks & 100M & 256\\
		seismic & seismic records & 100M & 256\\ 
		SALD & MRI data & 200M & 128\\ 
		deep1B & image descriptors & 267M & 96\\ 
		%iEEG & 4 in 5 & 33 & 256\\ 
	\end{tabular}
	\caption{Experimental datasets}
	\label{tab:datasets}
%	\vspace{-5pt}
\end{table}

\vspace{5pt} 
\noindent{\bf Measures.} We use the following measures to assess the estimation quality of each method and compare their results:

XXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXX

\vspace{5pt} 
\noindent\emph{Time Savings:} Given a load of queries and a stopping criterion, it measures the time saved as a percentage of the total time needed to complete the search without early stopping.

\vspace{5pt} 
\noindent{\bf Validation Methodology.} 
To evaluate the different methods, we use a Monte Carlo cross-validation approach that consists of the following steps. 
For each dataset, we randomly draw two disjoint sets of data series $\mathcal{W}_{pool}$ and $\mathcal{T}_{pool}$ and pre-calculate all distances between the series of these two sets. 
The first set serves as a pool for drawing random sets of witnesses (if applicable), while the second set serves as a pool for randomly drawing training (if applicable) and testing queries. 
At each iteration, we draw $n_w$ witnesses ($n_w=50$, $100$, $200$, or $500$) and/or $n_r$ training queries ($n_r=50$, $100$, or $200$) from $\mathcal{W}_{pool}$ and $\mathcal{T}_{pool}$, respectively. 
We also draw $n_t=200$ testing queries from $\mathcal{T}_{pool}$ such that they do not overlap with the training queries. We train and test the evaluated methods and then repeat the same procedure $N = 100$ times, where each time, we draw a new set of witnesses, training, and testing queries. 
Thus, for each method and condition, our results are based on a total of $N \times n_t = 20K$ measurements. %100 \times 200 = 20000$ test measurements.











\subsection{Results on XXXXXXXXXXXXX}
%\vspace{5pt} 





\subsection{Results on Time Savings}
We compare our stopping criteria (see Section~\ref{sec:stopping}) and assess the time savings they offer. 













==> new-intro.tex <==
\section{Introduction-New}
\label{sec:intro}

{\bf ???
- add experimental results, graphs

- add pseudocodes

- add discussion of kNN classifier variants (\url{https://en.wikipedia.org/wiki/K-nearest_neighbors_algorithm#The_weighted_nearest_neighbour_classifier}, and theoretical analysis of their accuracy/error rate (\url{https://en.wikipedia.org/wiki/K-nearest_neighbors_algorithm#Properties})
???}

\noindent
%\paragraph
\textbf{Data Series.} 
Data series are ordered sequences of values measured and recorded from a wide range of human activities and natural processes~\cite{Palpanas2019}, such as seismic activity, %per millisecond, human blood oxygen saturation, % per hour, 
or electroencephalography (EEG) signal recordings. % by putting hundreds of electrodes on the human scalp. 
The analysis of such sequences\footnote{If the dimension that imposes the ordering of the sequence is time then we talk about \emph{time series}. Though, a series can also be defined over other measures (angle in radial profiles in astronomy, mass in mass spectroscopy in physics, 
frequency in infrared spectroscopy in medicine, 
position in genome sequences in biology, 
etc.). We use the terms \emph{time series}, \emph{data series}, and \emph{sequence} interchangeably.} is becoming increasingly challenging as their sizes often grow to multiple terabytes~\cite{DBLP:journals/sigmod/Palpanas15,DBLP:journals/dagstuhl-reports/BagnallCPZ19}. 

Data series analysis involves pattern matching~\cite{DBLP:journals/pvldb/ZoumpatianosIP15,journal/vldb/linardi19}, anomaly detection~\cite{journal/csur/Chandola2009,journal/vldb/Dallachiesa2014,norma,series2graph}, frequent pattern mining~\cite{Rakthanmanon:2012:SMT,VALMOD}, clustering~\cite{conf/kdd/Keogh1998,conf/sdm/Rodrigues2006,conf/icdm/Keogh2011,journal/pattrecog/Warren2005}, and classification~\cite{journal/jmlr/Chen2009}. 
These tasks rely on \emph{data series similarity}. 
The data-mining community has proposed several techniques, %to automate such tasks,
%~\cite{Fu:2011}, 
including many similarity measures (or distance measure algorithms), for calculating the distance between two data series~\cite{Ding:2008,DBLP:conf/ssdbm/MirylenkaDP17}, as well as corresponding indexing techniques and algorithms~\cite{Echihabi:2018,evolutionofanindex}, in order to address scalability challenges.

\vspace{5pt} 
\noindent
%\paragraph
\textbf{Data Series Similarity.} 
We observe that data series similarity is often domain- and visualization-dependent~\cite{Batista:2014:CEC,Gogolou:2019}, and in many situations, analysts depend on time-consuming manual analysis processes.
For example, neuroscientists manually inspect the EEG data of their patients, using visual analysis tools, so as to identify patterns of interest~\cite{Jing:2016,Gogolou:2019}.
In such cases, it is important to have techniques that operate within interactive response times~\cite{resp-times}, in order to enable analysts to complete their tasks easily and quickly.

Both the data management and the human-computer interaction communities have studied the problem of how to use time series similarity in order to perform effective time series search. 
In the past years, several visual analysis tools have combined visualizations with advanced data management and analytics techniques (e.g.,~\cite{Rahman:2017:ISE,DBLP:journals/pvldb/Kraska18}), albeit not targeted to data series similarity search. 
Moreover, we note that even though the data series management community is focusing on scalability issues, % related to the processing and analysis of very large sequence collections, 
the state-of-the-art indexes currently used for scalable data series processing~\cite{Wang:2013:DDS,journal/kais/Camerra2014,Zoumpatianos:2016,journal/pvldb/kondylakis18,journal/vldb/linardi19} are still far from achieving interactive response times~\cite{Echihabi:2018,conf/vldb/echihabi2019}. 


\begin{figure}[tb]
\centering
\footnotesize
%\vspace{-5pt}
\includegraphics[width=0.94\linewidth]{motivation-normalized.pdf}
%\vspace*{-8pt}
\caption{Progression of the $1$-NN distance error (Euclidean distance) for 4 example queries (seismic dataset)~\cite{progressive1nn}, using the iSAX2+ index~\cite{journal/kais/Camerra2014}. The points in each curve represent approximate (intermediate points) or exact answers (last point) given by the algorithm. The lines end when the similarity search ends. The thick grey line represents the average trend over a random sample of 100 queries.}
\label{fig:motivation}
%\vspace*{-0.4cm}
\end{figure}


\vspace{5pt} 
\noindent
%\paragraph
\textbf{Progressive Results.} 
To allow for interactive response times when users analyze large data series collections, we need to consider progressive and iterative visual analytics approaches~\cite{Badam:2017,Zgraggen:2017,Turkay:2017,DBLP:conf/edbt/GogolouTPB19}. 
Such approaches provide progressive answers to users' requests~\cite{Fisher:2012,Stolper:2014,Moritz:2017}, sometimes based on algorithms that return quick approximate answers~\cite{Ding:2016,Fekete:2016}. 
%~\cite{Ciaccia:2000, Ding:2016, Fekete:2016}. 
Their goal is to support exploration and decision making by providing progressive (i.e., intermediate) results, before the final and exact ones have been computed. 
Most of the above techniques consider approximations of aggregate queries on relational databases, with the exception of Ciaccia et al.~\cite{Ciaccia:1999,Ciaccia:2000}, who provide a probabilistic method for assessing how far an approximate answer is from the exact answer.
%(up to 100 dimensions). 
Nevertheless, these works do not consider data series that are high-dimensional: their dimensionality (i.e., number of points in the series~\cite{Echihabi:2018}) ranges from several hundreds to several thousands. % (the dimensionality of a data series is defined \changed{by its number of points~\cite{Echihabi:2018}).}%, i.e., the number of points in the series). 
We note that the framework of Ciaccia et al.~\cite{Ciaccia:1999,Ciaccia:2000} does not explicitly target progressive similarity search. 
Furthermore, the approach has only been tested on datasets with up to 275K vectors with dimensionality of a few dozen, while we are targeting data series vectors in the order of hundreds of millions with dimensionality in the order of hundreds (the dimensionality of a data series is defined by its length~\cite{Echihabi:2018}, i.e., the number of points in the series). 
Our experiments show that the probabilistic estimates that their methods~\cite{Ciaccia:1999,Ciaccia:2000} provide are inaccurate and cannot support progressive similarity search.

In this study, we demonstrate the importance of XXXXX
Our results show that XXXXX

In our previous work, we established that there is a large gap between the time the 1st Nearest Neighbour (1-NN) is found and the time when the search algorithm terminates, i.e., users often wait without any improvement in their answers~\cite{DBLP:conf/edbt/GogolouTPB19,progressive1nn}. 
Figure~\ref{fig:motivation} presents the approximate results of the iSAX2+ index~\cite{journal/kais/Camerra2014} for four example queries on a 100M data series collection with seismic data~\cite{url/data/seismic}, where we show the evolution of the approximation error as a percentage of the exact $1$-NN distance.
We observe that the algorithm provides approximate answers within a few milliseconds, and those answers gradually converge to the exact answer, which is the distance of the query from the $1$-NN. 
Interestingly, the $1$-NN is often found in less than 1 sec (e.g., see yellow line), but it takes the search algorithm much longer to verify that there is no better answer and terminate. 
This finding is consistent with previously reported results~\cite{Ciaccia:2000,DBLP:conf/edbt/GogolouTPB19}, who report that most of the time spent in an exact NN search is ''wasted time, during which no improvement is obtained.'' 

Several similarity-search algorithms, such as the iSAX2+ index~\cite{journal/kais/Camerra2014} and the DSTree~\cite{Wang:2013:DDS} (the two top performers in terms of data series similarity search~\cite{Echihabi:2018}), provide very quick approximate answers. In this paper, we argue that such algorithms can be used as the basis for supporting progressive similarity search.  Unfortunately, these algorithms do not provide any guarantees about the quality of their approximate answers, while our goal is to provide such guarantees. 

\vspace{5pt} 
\noindent
\textbf{Proposed Approach.} 
We develop the first progressive approaches for data series similarity search with probabilistic quality guarantees, which are scalable to very large data series collections.  
Our goal is to predict how much improvement is expected when the search algorithm is still running. 
Communicating this information to users will allow them to terminate a progressive search early and save time.

The challenge is how to XXXXXXXX
Our approach consists in XXXXXXX



\vspace{5pt} 
\noindent
%\paragraph
\textbf{Contributions.} 
Our key contributions are summarized as follows.
\begin{itemize}
\item 
%\noindent$\bullet$
We formulate XXXXXXXX
\item 
%\noindent$\bullet$
We investigate XXXXXXXX
\item
%\noindent$\bullet$
Based on the above bounds, we further develop XXXXXXXXXX
\item
%\noindent$\bullet$
We perform an extensive experimental evaluation\footnote{The source code and datasets used in this paper are provided in~\cite{?????}.} with both synthetic and real datasets, comparing our solutions to existing baselines. 
The results demonstrate that our solutions XXXXXXXXX
\end{itemize}

%{\color{red}REVIEWER: The work is more of a delta research. There are tons of work on time series data and similarity queries, including the authors' prior work, and there is also tons of work on progressive queries. This paper kind of merging these two lines of work.}
% 
%{\color{red}REVIEWER: Throughout the whole paper, the author refers to [14,15] as state-of-the-art techniques. Experiments also compare with and discuss in details [14,15]. These two references are 20-years old ones published in ADC 1999 and ICDE 2000. I wonder why there was no other work in this area for the last 20 years.}
%
%{\color{red}REVIEWER: In the introduction, the paper lists four contributions. I do not see that the first two contributions should be counted. Progressive query answer has been there for long, and their importance are well known, regardless of the query type. So, introducing the problem of progressive similarity search would not be a contribution as similarity search is just another query that would benefit from progressive answer, same like other queries. Also, demonstrating the importance of such queries is not a contribution. It is your motivation for the paper.}
%
%{\color{red}REVIEWER: Weak/Conflicting Motivation: The goal of progressive or adaptive querying techniques (e.g. ADS) is to help scientists query series data as soon as possible without having to wait for the entire index to be built. This is useful mainly because of 2 reasons: 1) in some time critical scenarios, analysts/scientists don’t have time to wait for the entire index to be built in order to answer handful of queries, and 2) in tasks such as exploration, scientists may need to query a few regions to first determine whether to even look deeper into that particular column/series of data. Thus, the querying (including indexing) has to be “extremely fast”. On the other hand, the proposed approach requires training the models using hundreds of queries (which requires time in hours on a well-equipped Dell T630 rack server). In my opinion, this is contradictory to the motivation and goal of the progressive k-NN querying techniques. }
%{\bf ??? our argument: we index offline (takes lots of time), we spend a little bit extra time to train (again offline), then we are ready to support the online data exploration part that involves running many queries and we want to support *online* interactions ???}
%
%{\color{red}REVIEWER: The proposed method is largely built upon other existing works. I am not impressed with their techniques or derivation.}
%
%{\color{red}REVIEWER: The progressive estimation depends on an important observation that the approximate answers of index-based algorithms are close to the exact answers. However, this is one key point that this paper criticizes in the beginning (other progressive computation mechanisms may generate results that fluctuate). It seems to me that the linear models that are proposed are a simple generalization of what they observe. It just confirms that existing works on progressive similarity search using indexed approach work.}

\vspace{5pt} 
\noindent
%%\paragraph
\textbf{Paper Structure.} 
The rest of this paper\footnote{A preliminary version of this paper has appeared elsewhere~\cite{progressive1nn}.} is organized as follows. 
Section 2 summarizes related work on data series similarity search and progressive visual analytics. Section 3 presents background terminology. 
Section 4 defines progressive similarly search and introduces the main concepts for supporting prediction with probabilistic guarantees. 
Section 5 describes existing and new methods that we use to estimate a $k$-NN distance before and during the execution of a similarity search query. 
Section 6 presents an extensive evaluation of these methods. 
Section 7 illustrates how to apply our approach to help users evaluate the progressive results of similarity search. 
Finally, Section 8 concludes the paper and proposes directions for future work.
{\bf ??? check if correct, replace section numbers with section references ???}




==> new-preliminaries.tex <==
\section{Preliminaries and Background-New}\label{sec:def}

%\subsection{Data Series Similarity Search}

%Echihabi et al.~\cite{Echihabi:2018} offer a common language to describe data series similarity search. Our definitions are largely based on their terminology. 

%\vspace{5pt} 
\noindent{\bf Data Series and Data Series Collections:} 
A \textit{data series} $S(p_1,p_2,...,p_\ell)$ is an ordered sequence of points with length $n$.
% Similarly, a \textit{subsequence} $S[i:j]$ is the sequence $S(p_i,p_{i+1},...,p_{j-1},p_j)$, where $1 \leq i \leq j \leq \ell$. 
%In this paper, we only examine \textit{univariate series}, where each point in the series is scalar, i.e., it represents the value of a single variable.
A data series of length $\ell$ can also be represented as a single point in an $\ell$-dimensional space. For this reason, the values of a data series are often called \emph{dimensions}, and its length $\ell$ is called \emph{dimensionality}.
%
%\vspace{5pt} 
%\noindent{\bf Data Series Collections:} 
We use $\mathbb{S}$ to denote a \textit{data series collection} (or \textit{dataset}). 
We refer to the size $n=|\mathbb{S}|$ of a data series collection as \textit{cardinality}. 
In this paper, we focus on datasets with very large numbers of data series.
%A data series dataset $\mathbb{S}$ can be seen as a random sample taken from a large or infinite population of data series $\mathcal{U}$. 
%Being a random sample, the dataset is expected to be representative of the population. 
%Likewise, we can take a random sample of a dataset to produce a smaller dataset. 

\vspace{5pt} 
\noindent{\bf Distance Measures.} A data series \textit{distance} $d(S_1,S_2)$ is a function that measures the dissimilarity of two data series $S_1$ and $S_2$, or alternatively, the dissimilarity of two data series subsequences. 
As mentioned in Section~\ref{sec:related-work}, we chose Euclidean Distance (ED) as a measure due to its popularity and efficiency~\cite{Ding:2008}. % for large datasets~\cite{Ding:2008}.

%Ding et al.~\cite{Ding:2008} discuss a range of distance functions. Euclidean Distance (ED) is the most popular, performing point-by-point value comparison between two time series. ED can be combined with data normalization, often \emph{z-normalization}, considering as similar patterns that may vary in amplitude or value offset. Based on their analysis, Ding et al.~\cite{Ding:2008} concluded that there is no superior measure. In our work, we focus on ED because~\cite{Ding:2008,Echihabi:2018}: (i) it is an effective and the most commonly used measure in the visualization and data-mining literature; (ii) it leads to efficient solutions for large datasets. We plan to examine other measures, e.g., Dynamic Time Warping (DTW), in our future work.

\vspace{5pt} 
\noindent{\bf Similarity Search Queries.}
Given a dataset $\mathbb{S}$, a \textit{query} series $Q$, and a distance function $d(\cdot,\cdot)$, a \textit{k-Nearest-Neighbor (k-NN) query} identifies the $k$ series in the dataset with the smallest distances to $Q$. The 1st Nearest Neighbor (1-NN) is the series in the dataset with the smallest distance to $Q$.

%Although other types of queries exist, such as \textit{r-range} queries, we do not address them here. We further simplify our presentation by focusing on \textit{whole-matching queries}. As Echihabi et al.~\cite{Echihabi:2018} explain, \textit{subsequence-matching} queries can be trivially converted to whole matching queries. 
%{\color{red}REVIEWER: Section 3, page 3: What are "whole-matching queries" and "subsequence-matching queries"? They are not defined or explained.}

Similarity search can be \textit{exact}, when it produces answers that are always correct, or \textit{approximate}, when there is no such strict guarantee. 
%Echihabi et al.~\cite{Echihabi:2018} identify different flavors of approximate similarity search algorithms, based on what types of ''soft'' guarantees (probabilistic or relative distance error bounds) they provide. 
%In particular, a 
A \textit{$\delta$-$\epsilon$-approximate algorithm} guarantees that its distance results will have a relative error no more than $\epsilon$ with a probability of at least $\delta$~\cite{Echihabi:2018}. 
We note that only a couple of approaches~\cite{Arya:1998,Ciaccia:2000} provide such guarantees. 
Yet, their accuracy has never been tested on the range of dimensions and dataset sizes that we examine here. 

\vspace{5pt} 
\noindent{\bf Similarity Search Methods.} 
Most data series similarity search techniques~\cite{conf/sigmod/Faloutsos1994,Ciaccia:1998:CMS,Wang:2013:DDS,Camerra:2010:IIM,Zoumpatianos:2016,dpisaxjournal,conf/bigdata/peng18,journal/pvldb/kondylakis18,journal/vldb/linardi19} use an index, which enables scalability.
The index can offer quick approximate answers by traversing a single path of the index structure to visit the single most promising leaf, from where we select the \textit{best-so-far (bsf)} answer: this is the candidate answer in the leaf that best matches (has the smallest distance to) the query. 
The bsf may, or may not be the final, exact answer: in order to verify, we need to either prune, or visit all the other leaves of the index. 
%In this process, 
Having a good first bsf (i.e., close to the exact answer) leads to efficient pruning. % of the search space.

In the general case, approximate data series similarity search algorithms do not provide guarantees about the quality of their answers. 
In our work, we illustrate how we can efficiently %and effectively 
provide such guarantees, with probabilistic bounds. 

We focus on index-based approaches that support both quick approximate, and slower but exact, similarity search results. 
%In this work, we adapt the state-of-the-art ADS index~\cite{Zoumpatianos:2016}, which finds high-quality approximate answers almost immediately, and subsequently updates these answers that converge fast to the final, exact answer. 
%We also adapt the DSTree index~\cite{Wang:2013:DDS}, which has been shown to answer queries very fast~\cite{Echihabi:2018}, and demonstrate the applicability of our techniques to this index, as well. 
In this work, we adapt the state-of-the-art data series indexes iSAX2+~\cite{journal/kais/Camerra2014} and DSTree~\cite{Wang:2013:DDS}, which have been shown to outperform the other data series methods in query answering~\cite{Echihabi:2018}, and we demonstrate that our techniques are applicable to both indexes. 
We provide below a succinct description of the iSAX2+ and DSTree approaches.

The iSAX2+~\cite{journal/kais/Camerra2014} index organizes the data in a tree structure, where the leaf nodes contain the raw data and each internal node summarizes the data series that belong to its subtree using a representation called \textit{Symbolic Aggregate Approximation (SAX)}~\cite{conf/dmkd/LinKLC03}. SAX transforms a data series using Piecewise Aggregate Approximation (PAA)~\cite{journal/kais/Keogh2001} into equi-length segments, where each segment is associated with the mean value of its points, then represents the mean values using a discrete set of symbols for a smaller footprint. 

%Similarly to iSAX2+, the 
DSTree~\cite{Wang:2013:DDS} is also a tree-based index that stores raw data in the leaves and summaries in internal nodes. 
Contrary to iSAX2+, DSTree does not support bulkloading, intertwines data segmentation with indexing and uses \textit{Extended Adaptive Piecewise Approximation (EAPCA)}~\cite{Wang:2013:DDS} instead of SAX. With EAPCA, a data series is segmented using %{\it Adaptive Piecewise Constant Approximation}
APCA~\cite{journal/acds/Chakrabarti2002} into varying-length segments, then each segment is represented with its mean and standard deviation values.

Since the query answering time depends on the data distribution~\cite{conf/kdd/Zoumpatianos2015}, and both iSAX2+ and DSTree can produce unbalanced index trees, we provide below an index-invariant asymptotic analysis on the lower/upper bounds of the query runtime. 
As we consider large on-disk datasets, the query runtime is I/O bound; thus we express complexity in terms of I/O~\cite{analysis-kanellakis,analysis-hellerstein}, using the dataset size $N$, the index leaf threshold $th$ and the disk block size $B$. 
Consider an index over a dataset of size $N$ such that each index leaf contains at most $th$ series ($th \ll N$). 
We count one disk page access of size $B$ as one I/O operation (for simplicity, we use $B$ to denote the number of series that fit in one disk page). 
Note that both the iSAX2+ and DSTree indexes fit the entire index tree in-memory; the leaves point to the raw data on-disk.

\underline{Best Case}. The best case scenario occurs when one of the children of the index root is a leaf, containing one data series,  which is the exact answer. 
In this case, the approximate search will incur $\Theta(1)$ I/O operation and will return the exact result. 
In the best case, exact search will prune all other nodes of the index and thus will also incur $\Theta(1)$ disk access. 
Note that a leaf is visited only once and that we do not account for the cost of visiting and pruning internal nodes because both operations occur in-memory.

\underline{Worst Case}. Approximate search always visits one leaf. 
Therefore, the worst case occurs when the leaf is the largest possible, i.e., it contains $th$ series, in which case approximate search incurs $\Theta(th/B)$ I/O operations. 
For exact search, the worst case occurs when the algorithm needs to visit every single leaf of the index. 
This can happen when the index tree has $N-th+1$ leaves (i.e., each leaf contains only one series, except for one leaf with $th$ series), as a result of each new series insertion causing a leaf split where only one series ends up in one of the children. 
Therefore, the exact search algorithm will access all the leaves, (except the one visited to find the first approximate answer) 
and will incur $\Theta(N)$ I/O operations. 
(Note that this is a pathological case that would happen when all series are almost identical, which prevents the splitting operation from distributing them evenly into separate leaves. 
In such a case, indexing and similarity search are not useful anyways.)

%Since the query answering time depends on the data distribution~\cite{conf/kdd/Zoumpatianos2015}, we provide below an asymptotic analysis %focused on the lower and upper bounds  of the iSAX2+ and DSTree query runtime. Note that both approaches can produce unbalanced index trees. Consider an index that contains $N$ series of length $t$ stored in $l$ leaves, with at most $th$ series in each leaf ($th \ll N$), and summarizes the data using $w$ segments and $s$ bits per segment.

%\underline{Best Case} (the index tree is balanced): In the case of iSAX2+, the series are divided equally among all the root children and the root subtrees are balanced and have equal height. Therefore, each subtree will contain $\lceil \frac {N} {th} \rceil / 2^w$ leaves. Finding the first approximate answer will require $\theta(\log_{2}({\lceil \frac {N} {th} \rceil / 2^w}))$  in-memory accesses and 1 disk read of size $\theta(th)$ (i.e., the leaf node). Exact search will incur this cost in addition to $2^w$ in-memory accesses to prune the root subtrees. As for the DSTree, the binary tree index will be balanced with a total of $\lceil \frac {N} {th} \rceil$ leaves. Approximate search will require $\theta(\log_{2}({{\lceil \frac {N} {th} \rceil}}))$ in-memory accesses and 1 disk read of size $\theta(th)$ to find the first approximate answer, and 1 additional in-memory access for exact search to prune the root node. {\bf ??? prune the *index root* node? ???} 

%\underline{Worst Case} (the index tree degenerates to a linked list): All the series are stored in one big leaf of size $N$. To find the first approximate answer, iSAX2+ will incur $\theta(w(s-1))$  in-memory accesses and 1 disk access of size $\theta(N)$, while DSTree will need $\theta(log_{2}(t))$ in-memory accesses and 1 disk access of size $\theta(N)$. In the worst case, exact search with both the DSTree and iSAX2+ will require visiting all the leaves of the index using random disk accesses. {\bf ??? but you said that the worst case index has 1 leaf of size N, there are no random accesses to multiple leaves ???}

% can provide very quick approximate answers by traversing a single path of the index structure to visit the most promising leaf. Such approximate answers provide a baseline \textit{best-so-far (bsf)} match. They define a lower-bounding distance that can be used to prune the   

\vspace{5pt} 
\noindent{\bf Progressive Similarity Search.}
We briefly describe here the progressive similarity search approach that we developed in our previous work~\cite{progressive1nn}.
XXXXXXXXXXXXXXXXXXXXXXX

Table~\ref{SymbolTable} summarizes the notation we use in this paper.

\begin{table}[tb]
\centering
\caption{Table of symbols}
%\vspace{-8pt}
%\vspace{2pt}
\label{SymbolTable}
\scalebox{0.88}{
\hspace{-0.6cm}
\begin{tabular}{r|l}
%\hline
{\bf Symbol} & {\bf Description} \\
\hline
$S$, $Q$					& data series, query series \\
%$S[i:j]$					& series subsequence from $i$ to $j$\\ 
$\ell$						& length of a data series \\
$\mathbb{S}$				& data series collection (or dataset)\\
$n=|\mathbb{S}|$			& number of series in $\mathbb{S}$ \\
$R(t)$						& progressive answer at time $t$ \\
%$Q$							& query series \\
\emph{k-NN}, $knn(Q)$		& $k^{th}$ Nearest Neighbor of $Q$ \\
$d_{Q,R}(t)$, $d(Q,R(t))$		& distance between $Q$ and $R(t)$\\
$d_{Q,knn}$, $d(Q,knn(Q))$				& distance between $Q$ and its \emph{k-NN} \\
${\epsilon}_Q(t)$			& relative distance error of $R(t)$ from \emph{k-NN} \\
$p_{Q}(t)$				& probability that  $R(t)$ is exact (i.e., the \emph{k-NN})\\
$t_{Q}$					& time to find the \emph{k-NN}\\
$\tau_{Q,\phi}$				& time to find the \emph{k-NN} with probability $1 - \phi$\\
$\tau_{Q,\theta,\epsilon}$ 		& time for which ${\epsilon}_Q(t) < \epsilon$ with confidence $1-\theta$\\
$\hat{\bullet}$				& estimate of $\bullet$ \\
$I_Q(t)$					& information at time $t$ \\
$h_{Q,t}(x)$				& probability density function of Q's distance \\
							& from its $k$-NN, given information $I_Q(t)$\\
$H_{Q,t}(x)$				& cumulative distribution function of Q's\\
							& distance from its $k$-NN, given $I_Q(t)$\\
$f_Q(x)$					& probability density function of $Q$'s distance \\
							& from a random series in $\mathbb{S}$ \\
$F_Q(x)$					& cumulative distribution function of $Q$'s\\
							&  distance from a random series in $\mathbb{S}$\\ 
$G_{Q,n}(x)$				& cumulative distribution function of $Q$'s\\
							& distance from its $k$-NN\\
$\mathcal{W}$				& set of witness series \\
$n_w=|\mathcal{W}|$			& number of witnesses in $|\mathcal{W}|$ 
%\hline
\end{tabular}
}
\end{table}
%\vspace{30pt}






==> new-related.tex <==
\section{Related Work-New}
\label{sec:related-work}
We now discuss previous work on time series similarity, interactive querying, and progressive visual analytics.

\vspace{5pt} 

%We describe next related work both from the data-base community on similarity search and querying, and work on progressive visual analytics.

%\vspace{5pt}
\noindent\textbf{Similarity Search.} % made a subsection of both Similarity Measures and Similarity Search
%\textbf{Similarity Measures:}
%
Several measures have been proposed for computing similarity between data series~\cite{Ding:2008,DBLP:conf/ssdbm/MirylenkaDP17}. 
Among them, Euclidean Distance (ED)~\cite{conf/sigmod/Faloutsos1994}, which performs a point-by-point value comparison between two time series, is one of the most popular. ED can be combined with data normalization (often \emph{z-normalization}~\cite{Goldin:1995:SQT}), in order to consider as similar patterns that may vary in amplitude or value offset. 
%Another common measure is Dynamic Time Warping (DTW)~\cite{Berndt:1994:UDT}, which allow temporal "stretching" or "compression" of a time series when searching for similar ones.
%Data-mining research proposed a plethora of similarity measures that compute similarity between time series. 
%Ding et al. ~\cite{Ding:2008} group measures that compute similarity between time series in four categories. Euclidean Distance (ED) ~\cite{conf/sigmod/Faloutsos1994} is the simplest one and belongs to \emph{Lock-step} measures, which perform point-by-point value comparison between time series. ED can be combined with data normalization, often \emph{z-normalization} ~\cite{Goldin:1995:SQT}, considering as similar patterns that may vary in amplitude or value offset. Another common category is \emph{Elastic} measures, such as Dynamic Time Warping (DTW) ~\cite{Berndt:1994:UDT}, which allow temporal "stretching" or "compression" of a time series when searching for similar ones. These measures account for similar sequences that may vary in speed or temporal shift. Other categories include \emph{threshold-based} measures, such as TQuEST ~\cite{Assfalg:2006:SST}, or \emph{pattern-based} measures, such as SpADe ~\cite{Chen:2007:SpADe}. To evaluate similarity measures, Ding et al. ~\cite{Ding:2008} compared the 1-NN classification accuracy of nine different similarity measures using several, different time series datasets with known, pre-labeled classes ~\cite{UCRArchive}. 
Ding et al.~\cite{Ding:2008} conducted an analysis of different measures (including elastic ones such as Dynamic Time Warping~\cite{Berndt:1994:UDT} and threshold based ones such as TQuEST ~\cite{Assfalg:2006:SST}) and concluded that there is no superior measure.
%, as their classification accuracy depends on the dataset and its domain. Among their findings is that, 
%On small datasets, DTW can be significantly more accurate than ED, but, as the size of the dataset increases their accuracies converge.
In our work, we focus on ED because~\cite{Ding:2008,Echihabi:2018} it is effective, it leads to efficient solutions for large datasets, and is 
%very commonly used. 
the most common distance measure in the visualization and data-mining literature.
 
%\anab{Fanis Ok? If so remove $=>$} Nevertheless, in our approach we could substitute ED by any other similarity distance measure. 
%%\anna{having similar accuracy with the most expensive Dynamic Time Warping (DTW). However, in our future experiments we are going to test how DTW results perform in the case of iterative analytics compared to ED}.
%\anab{ToDo: Move to future work $=>$ We plan to examine other measures, e.g., Dynamic Time Warping (DTW) in our future work.}
%; and (iii) it is appropriate for our research problem, because it satisfies the triangular inequality~\cite{Ciaccia:2000}. \anab{Anna why is (iii) important, do you explain it anywhere?} 
%Nevertheless, we note that in our process ED can be replaced by any other similarity measure that satisfies the triangular inequality. 

%\anna{This paragraph may go out!} 
The human-computer interaction community has focused on the interactive visual exploration and querying of data series. %They have even developed algorithmic similarity search methods by focusing on the visual characteristics of the patterns. 
%%\anab{Anna add here some refs on iterative visual search systems}
%%For example through the automatic detection of specific high-frequent, simple shapes such as spikes or valleys that users can combine to form queries ~\cite{17358} or through the automatic extraction of a grammar to express time series approximately and simplify the search of matches ~\cite{Muthumanickam:2016:SGE}. 
%%These works mainly perform visual matching of series and they have not been tested for their scalability to millions of data series. As a result, we cannot use them under the probabilistic-approach of our progressive similarity search work (Sec.~\ref{sec:research-strategy}), because they do not rely on the real values of data, but rather on their visual patterns \anna{Is that correct?}\anab{Who are you asking?}. %Another interesting direction of research from the human-computer interaction community is 
%In particular, they are interested in how to form interactive similarity search queries.
These querying approaches are visual, often on top of line chart visualizations~\cite{Tufte:1986:VDQ}, and rely either on the interactive selection of part of an existing series (e.g.,~\cite{Buono:2008:ISS}), or on sketching patterns to search for (e.g.,~\cite{Correll:2016,Mannino:2018:ETS}). 
%~\cite{Correll:2016, Holz:2009:RST, Mannino:2018:ETS, Siddiqui:2016:EDE, Wattenberg:2001:SGQ}. 
%These works mainly perform visual matching of series and have not been tested for their scalability to millions of data series. 
%Although we do not study mechanisms of querying in this paper, 
This line of work is orthogonal to our approach, which considers approximate and progressive results from these queries when interactive search times are not possible. 
%useful for our research, because we want to understand how people assess similarity in the results of their queries. 



%\vspace{5pt} 
%\noindent
%\paragraph
%\textbf{Similarity Search and Interactive Querying:}
%
\vspace{5pt}
\noindent
\textbf{Optimized and Approximate Similarity Search.} % made a subsection of both Similarity Measures and Similarity Search
The data-base community has optimized similarity search methods by using index structures~\cite{Beckmann:1990:RER,conf/sigmod/Faloutsos1994,Ciaccia:1997:MEA,Ciaccia:1998:CMS,Ferhatosmanoglu:2000:VAB,Wang:2013:DDS,Camerra:2010:IIM,Schafer:2012:SSF,Zoumpatianos:2016,dpisaxjournal,conf/bigdata/peng18,journal/pvldb/kondylakis18,journal/vldb/linardi19,parisplus,messi,ulissejournal}, 
or fast sequential scans~\cite{Rakthanmanon:2012:SMT,Yeh:2018:TSJ,Kashyap:2011:SKS}. 
Recently, Echihabi et al.~\cite{Echihabi:2018,url/DSSeval2} compared the efficiency of these methods under a unified experimental framework, showing that there is no single best method that outperforms all the rest.
%Each one of them has its pros and cons, which depends on a combination of factors, such as dataset size, time series length, disk-resident or in-memory search. Future work aims to combine the strengths and positive characteristics of the best methods in order to create the time series "mega-index".
%In our work, we use the state-of-the-art iSAX2+~\cite{journal/kais/Camerra2014} and DSTree~\cite{Wang:2013:DDS} indices, which provide high-quality approximate answers almost immediately, and then provide updates that converge fast to the exact answer. 
%\anna{We cannot utilize optimized sequential scan solutions like UCR Suite~\cite{Rakthanmanon:2012:SMT}, because they do not guarantee high-quality approximate results like index structures do.}
In this study, we focus on the popular centralized solutions, though, our results naturally extend to parallel and distributed solutions~\cite{conf/bigdata/peng18,parisplus,messi,dpisaxjournal}, % that have recently appeared in the literature~\cite{conf/bigdata/peng18, parisplus, dpisaxjournal}, 
since these solutions are based on the same principles and mechanisms as their centralized counterparts~\cite{evolutionofanindex}.
Moreover, we focus on (progressive answers for) exact query answering. 
Given enough time, all answers we produce are exact, which is important for several applications~\cite{Palpanas2019}. 
In this context, progressive answers help to speed-up exact queries by stopping execution early, when it is highly probable that the current progressive answer is the exact one.
%, e.g., when it is obvious from a progressive answer that a query does not lead to an interesting result. 
%In such cases, different analysts may employ different criteria (eg, [c]) that may terminate a search soon, late, or not at all. (Note that existing approximate answer methods either are not accurate [15,16] (Fig8), or require to create a new index for each different accuracy level~\cite{url/DSSeval2}, which is not amenable to progressive query answering.) 
%Moreover, our approach is good both for quick approximate results (with a controlled distance error), and for stopping early with a high probability of having the exact 1NN answer (Fig16left). So it is also relevant to users interested in quick exact answers. (Consider that the 1NN answer is often found long before the full search completion). 

In parallel to our work, Li et al.~\cite{msearlytermination} proposed a machine learning method, %based on gradient boosting decision trees, 
developed on top of inverted-file (IVF~\cite{DBLP:journals/pami/JegouDS11} and IMI~\cite{DBLP:journals/pami/BabenkoL15}) and k-NN graph (HNSW~\cite{DBLP:journals/pami/MalkovY20}) similarity search techniques, that solves the problem of early termination of approximate NN queries, while achieving a target recall. 
In contrast, our approach employs similarity search techniques based on data series indices~\cite{journal/pvldb/echihabi2019}, and with a very small training set (up to 200 training queries in our experiments), provides guarantees with per-query probabilistic bounds along different dimensions: on the distance error, on whether the current answer is the exact one, and on the time needed to find the exact answer.

XXXXXXXXXXXXXX

\vspace{5pt} 
\noindent
%\paragraph
\textbf{Progressive Analytics.}
progressive knn-classification, discord, other? 
{\bf ??? new references for progressive classification ???}

We may need to look previous work on approximate K-NN search:

\begin{enumerate}
\item \url{https://apacheignite.readme.io/docs/ann-approximate-nearest-neighbor}
\item \url{https://www.ijcai.org/Proceedings/11/Papers/222.pdf}
\item progressive classification based on multi-resolution object representations~\cite{DBLP:conf/icassp/CastelliLTK96}

\item \url{https://www.sciencedirect.com/science/article/abs/pii/S0306437905000128}
\end{enumerate}

XXXXXXXXXXXXXXXXXX

\vspace{5pt} 
\noindent
%\paragraph
\textbf{Progressive Visual Analytics.}
%%
%%This field is the intersection of database and human-computer interaction communities. 
%%More recent works~\cite{TODO} {\bf ??? missing references ???} combine the state-of-the-art of both domains and discuss how they 
%A recent research direction studies the problem of how we can support interactive, real-time visual analytics when back-end computations cannot be performed instantaneously, as is the case of our work. 
%%The need for scalable analytics and scalable interactive visualizations emerges due to the massive production and collection of data. 
%%These works utilize 
%To this effect we can use 
%progressive and iterative methods in order to produce fast, but approximate, computational results and visualizations, % of large datasets \anab{not only, it can be other types of computations}
%that are refined over time with increasing precision. 
Fekete and Primet~\cite{Fekete:2016} provide a summary of the features of a progressive system; three of them are particularly relevant to progressive data series search: 
%(i) provide increasingly meaningful partial results as the algorithm executes; (ii) provide feedback about the aliveness, absolute and relative progress of the computation; and (iii) guarantee time bounds in the delivery of progressive results. 
(i) progressively improved answers; (ii) feedback about the computation state and costs; and (iii) guarantees of time and error bounds for progressive and final results.
%We address these features in Section {\bf ??? fill in! do we even do this? ???}.
%
%The state-of-the-art in big data exploration takes advantage of the power of distributed systems, indexing, and sampling methods, and different works utilize one or more of these methods in order to provide progressive results for different kinds of queries and data. 
%In relational databases for example, 
Systems that support big data visual exploration include Zenvisage~\cite{Siddiqui:2016:EDE} that provides incremental results of aggregation queries, Falcon~\cite{Moritz:2019:FBI} that prefetches data for brushing and linking actions, and IncVisage~\cite{Rahman:2017:ISE} that %incrementally samples to 
progressively reveals salient features in heatmap and trendline visualizations. 

Systems that provide progressive results are appreciated by users due to their quick feedback~\cite{Badam:2017,Zgraggen:2017}. Nevertheless, there are some caveats. Users can be mislead into believing false patterns~\cite{Moritz:2017,Turkay:2017} with early progressive results. It is thus important to communicate the progress of ongoing computations~\cite{Angelini2018ARA,Schulz:2016:EVP}, including the uncertainty and convergence of results~\cite{Angelini2018ARA} and guarantees on time and error bounds~\cite{Fekete:2016}.  
Previous work provides such uncertainty and guarantees in relational databases and aggregation type queries~\cite{DBLP:conf/sigmod/HellersteinHW97,DBLP:journals/tods/JermaineAPD08,DBLP:series/isrl/WuOT13}.  
Fisher et al.~\cite{Fisher:2012:TMI} studied if analysts trust data that come from incremental samples with added statistical measures, such as means and confidence intervals built on a standard SQL database. 
Moritz et al.~\cite{Moritz:2017} used an existing algorithm~\cite{Ding:2016} that exploits sampling methods and approximate query processing for incremental, approximate aggregate database queries, communicating errors and confidence intervals. 
They evaluated with a user study how users assess the uncertainty of partial, numerical average results of flight-delay data and how the knowledge of these results guided their exploratory process and affected their decision making. 

Closer to the context of data series, Ciaccia and Patella~\cite{Ciaccia:2000} studied similarity search queries over general multi-dimensional spaces and proposed a probabilistic approach for computing the uncertainty of partial similarity search results. 
However, their approach does not scale to the dataset sizes and number of dimensions that we target. 
We discuss their approach in the following section.
%Their progressive similarity search algorithm exploits the M-tree index structure and approximate query processing. However, they did not evaluate their approach with a user study and they did not use data series. 
%\anab{Anna we are also not doing a user study, so do not use this as a critique. Also the second looks like it could work for timeseries (they are multidimensional data - why is their work not enough?)}


